In-Hand 3D Object Scanning from an RGB Sequence

We propose a method for in-hand 3D scanning of an unknown object with a monocular camera. Our method relies on a neural implicit surface representation that captures both the geometry and the appearance of the object, however, by contrast with most NeRF-based methods, we do not assume that the camera-object relative poses are known. Instead, we simultaneously optimize both the object shape and the pose trajectory. As direct optimization over all shape and pose parameters is prone to fail without coarse-level initialization, we propose an incremental approach that starts by splitting the sequence into carefully selected overlapping segments within which the optimization is likely to succeed. We reconstruct the object shape and track its poses independently within each segment, then merge all the segments before performing a global optimization. We show that our method is able to reconstruct the shape and color of both textured and challenging texture-less objects, outperforms classical methods that rely only on appearance features, and that its performance is close to recent methods that assume known camera poses.

==> 3_4old_bg_and_formulation.tex <==
\textvars{bg,col,seg,BCE,opf,reg,inc,trac,OF,dep}



\section{In-hand object scanning setup}
\label{sec:problem}

The setup for in-hand object scanning consists of a single RGB camera and an unknown rigid object being manipulated by one or two hands in the field of view of the camera. Our method relies on segmentation masks of the object which can be obtained from existing pre-trained networks that either work on a single RGB image~\cite{zhou2022detecting} or on a pair of images when the background is static~\cite{boerdijk2020learning}. As we aim to obtain reconstruction of only the object and not the hands, we additionally use segmentation masks from \cite{wu2021seqformer} to ignore the hand pixels in our method. We also assume that the object is far enough from the light sources and the camera such that the relative change in object's 3D location is small throughout the scanning. This assumption allows us to simplify the modeling of specular reflections on the object surface during scanning as explained in the next section.
Such an assumption is reasonable as rotation is the primary transformation of the object during in-hand scanning. On the HO-3D dataset, which contains sequences of a hand manipulating objects, the maximum standard deviation of the object's 3D location is only \shreyasrmk{XX}\,mm.


% which validates our assumption.

% Our setup for in-hand object scanning consists of a static RGB camera \tomasrmk{The camera needs to be static only to ensure static background, right? And static background is useful mostly for straightforward segmentation of the unknown object? We could formulate the problem without making any assumption on whether the camera is static and instead assume that the masks are available (and say that in our experiments we obtain the masks using the methods cited below).} and an unknown rigid object being handled by one or two hands in the field of view of the camera.
% We assume a static background whose image is either obtained separately or is estimated from the sequence using the segmentation masks of the hand and the object. \tomasrmk{The static background is required only by \cite{boerdijk2020learning} and not by any other component of our method -- is that correct? If so, I would propose to make it explicit that the static background requirement is coming from \cite{boerdijk2020learning}, and can be removed if the object masks are obtained using e.g. Detic -- this will be hopefully shown on the Aria sequences.}
% We use a pre-trained network from \cite{boerdijk2020learning} to segment the dynamic foreground and combine it with accurate hand segmentations obtained from \cite{wu2021seqformer} to obtain the masks of the hand, the object, and the background.

% \tomasrmk{I think the following should go to the Method section. "Problem Formulation" is typically definition of the task to solve, i.e., explaining what is the input, what is the output, what are constrains coming from the considered setup. "We represent the object surface using an occupancy field..." is already one specific approach that we took to solve the problem and should I think thus go to Method. Actually, I think it would be good to add also section "Preliminaries", where all the things specific to existing methods such as UNISURF would go.}

% \vincentrmk{I merged the 'background' and 'formulation' sections, because i felt it was too much text before reaching the actual method. I think having unisurf and our formulation together is good because it shows the differences/contributions compared to standard problems. Maybe 'Problem Formulation' is not a good name for the section, maybe 'Objective Function' or something similar?}

\section{Problem formulation}


We represent the object surface using an occupancy field and a color field inspired by UNISURF~\cite{unisurf}.
The occupancy field $o(.)$ of UNISURF is a mapping of the form:
%
\begin{equation}
    o_\theta(\bx): \mathbb{R}^3 \longrightarrow [0,1] \> ,  
\end{equation}
%
implemented with a deep network, where $\theta$ represents the parameters of the network and $\bx$ the 3D coordinates of a point in the object coordinate system. The object surface $\calS$ is represented by 3D points $\bx_\calS$ for which $o_\theta(\bx_\calS)=0.5$. The 3D mesh of the object can then be obtained from this implicit surface using the Marching Cubes algorithm~\cite{mcubes}.

The color field $c_\theta(\bx; \bd, \bn_\bx, \bh_\bx)$ in UNISURF is also realized by a deep neural network, represents the color at each 3D point and is conditioned on the viewing direction $\bd$, the normal $\bn_\bx$ at point $\bx$ and the geometry feature $\bh_\bx$ at point $\bx$. Note that to simplify the notations we include in $\theta$ both the parameters of the occupancy field and of the color field as these two networks are optimized together. Such a model accounts for the specular reflections on the object surface under the Phong reflection model~\cite{HughesDamEtAl13}. We propose to use the same color field model for the object during in-hand scanning as the object-light source distance is large compared to the variations in object's 3D position. As the object moves w.r.t light source during scanning, the observed color at a point on the surface of the object depends on the direction of incoming light, the viewing direction and direction of normal as the point. The direction of incoming light can be approximated to remain unchanged throughout the sequence as the relative change in 3D position of the object is small during scanning. Thus, the observed color depends only on the viewing direction and normal.


% As illustrated in Figure~\ref{fig:raydist}, such a model accounts for the specular reflections on the object surface under the Phong reflection model~\cite{HughesDamEtAl13} when the position of the light source w.r.t to the object is fixed. This is the standard setup for NeRF-based methods. However, in the case of in-hand scanning, the pose of the object varies wrt to the light sources. \shreyas{The color field thus also depends on the distance of the ray from the camera and is denoted by $c_\theta(\bx; \bd, \bn_\bx, \bh_\bx, p_\bx)$ where $p_\bx$ is distance between $\bx$ and the camera center. In practice, we observe that the relative distance of the object from the camera during in-hand scanning has little variations throughout the sequence. On the HO-3D dataset~\cite{hampali-cvpr20-honnotate} the maximum standard deviation of the object's distance from the camera is xx with a mean of xx\shreyasrmk{TODO}. Thus the influence of $p_\bx$ on the color field is negligible for these sequences.}\shreyasrmk{I feel this kind of a explanation is risky. What if we just state in the beginning of this section that we assume that the object is at a fixed distance from the camera during scanning. To justify the assumption we quote numbers from ho-3d dataset.} \tomasrmk{As we don't have numbers to support this contribution/story, I would remove this paragraph (also Figure 2). The Phong reflection model is violated in our setup because the object is not at a fixed distance from the light source, right? But since object-camera distance is typically $<<$ object-light distance, the small deviations of the object-light distance throughout the sequence probably don't influence much. Hence, I think we can just write that in this paper we model the surface reflectance using the Phone reflection model (+ we can add the explanation from the previous sentence to justify why this model is sufficient).}
% We thus condition the color field on the distance---which we denote $p_\bx$---between the camera center and 3D point $\bx$. 
% \vincentrmk{I am still confused, didnt your experiments show that $p$ has little influence?}

% The static pose between the object and the light source in all the images results in a constant incoming light radiance at any point on the object surface as shown in Figure~\ref{fig:static_object}.

% However, the varying position of the object w.r.t the light source results in varying incoming light radiance, $\omega_i$ on the object surface as illustrated in Figure~\ref{fig:static_camera} for the in-hand object scanning setup. Under the Phong reflection model~\cite{HughesDamEtAl13}, the observed radiance at a point on the object surface depends on the viewing direction, $\bd$, direction of the normal at the point, $\bn$ and the incoming light direction, $\omega_i$. As the relative position between the camera and the light source remains fixed, the incoming light direction can be parameterized as $\omega_i = f(\bx, \bd, \bn, p)$, where $p$ is the length of the viewing ray. $p$ is computed as the distance between the camera optic center and the 3D point at which the observed radiance is calculated. 

In UNISURF, the rendered color at a pixel in a frame $i$ is obtained by integrating the color values along the ray $\ray$ originating from the camera center and passing through the pixel. The continuous integration is approximated as:
%
\begin{gather}
    \hat{C}_i(\ray) = \sum_{k=1}^M \gamma(\bx_k) c_\theta(\bx_k, \bd, \bh_{\bx_k}, \bn_{\bx_k}, p_{\bx_k}) \>, \\
    \gamma(\bx_k) = o_\theta(\bx_k)\prod_{l<k}\big(1-o_\theta(\bx_l)\big) \nonumber \> ,
    \label{eq:rend_unisurf}
\end{gather}
%
where $\{\bx_k\}$ are $M$ samples along ray $\ray$. $\hat{C}_i(\ray)$ is the estimated colored in frame $i$ at pixel $\ray$, and $\gamma(\bx_k)$ is the estimated alpha-blending coefficient that evaluates to 1 if point $\bx_k$ is on the surface of the object and 0 otherwise. \shreyas{The ray $\ray$ is sampled from the entire image space and surrounding environment along with the object is reconstructed. In our case, we are not interested in reconstructing the background nor the hand. Hence, we sample the rays for rendering only from the object regions of the image which is obtained from the segmentation mask of the object.}\shreyasrmk{The background image was required only because the masks were not perfect. I propose to keep this small modification of $C(\ray)$ with background pixels as an implementation detail. If the masks were good (which it is in most scenarios), we did not have to worry about this. I think this way we can keep the explanation simple and also not emphasis on static camera}

\vincentrmk{I am not sure anymore if we need a $C_i(\ray)$ different from unisurf, besides the background?}


% We therefore modified the computation of 
% $\hat{C}_i(\ray)$ to include pixels from the background:
% %
% \begin{align*}
%     \hat{C}_i(\ray) &= \sum_{k=1}^M \gamma(\bx_k) c_\theta(\bx_k,\bd, p_k, \bn_{\bx_k}, \bh_{\bx_k}) + \gamma_\bg c_\bg(\ray) \> ,
% \end{align*}
% %
% where $\gamma_\bg$ is a blending coefficient computed as $\gamma_\bg = \prod_k\big(1-o_\theta(\bx_k)\big)$ to set the 
% colors of pixels where the corresponding ray $\ray$ does not intersect the reconstructed object to the color $c_\bg(\ray)$ of the background at this pixel.


% When the object masks are accurate, the background pixels in each image can be set to black color and original rendering equation in Eq.~(\ref{eq:rend_unisurf}) can be used. However, since the masks obtained from the segmentation network~\cite{boerdijk2020learning} are often noisy we use background pixels during rendering to mitigate the effect of inaccurate masks. 

% \begin{figure}
%     \centering
%     \begin{minipage}{0.35\linewidth}
%         \subcaptionbox{Two camera poses in Standard-NeRF setup\label{fig:static_object}}
%         {\includegraphics[page=1,width=1\linewidth,trim=10 150 620 115, clip,]{figures/method/ray_length.pdf}}
%     \end{minipage}~
%     \begin{minipage}{0.65\linewidth}
%         \subcaptionbox{Two object poses in in-hand object scanning setup\label{fig:static_camera}}
%         {\includegraphics[page=1,width=1\linewidth,trim=350 150 10 120, clip,]{figures/method/ray_length.pdf}}
%     \end{minipage}
%     \caption{\shreyas{(a) In standard-NeRF setting, the color field is a function of viewing ray direction and normal as the incident ray direction $\omega$ is fixed.  (b) In in-hand scanning scenario, the observed color depends on the pose of the object relative to the camera and the color field needs to be additionally conditioned on ray distance along with ray direction and normal.}}
%     % \caption{\shreyas{(a) In the case of the standard NeRF setting, the camera moves with respect to the object, and the observed radiance at a 3D point depends only on the viewing ray direction and the normal as the incident light direction is fixed in all frames. (b) In the case of in-hand scanning, the object moves with respect to the fixed camera and the lights setup, and the incident light direction at a 3D point on the surface of the object depends on the camera-object relative pose. To capture this, we simply condition the radiance on the distance between the camera and the point (ray length), in addition to the direction of the viewing ray and normal.}}
%     \label{fig:raydist}
% \end{figure}



UNISURF estimates the network parameters by minimizing the photometric loss
%
\begin{gather}
    \theta^* = \arg\min_\theta \sum_i \sum_{\ray \in \calR_i} \loss_{\text{col}}^i(\ray) \nonumber \> ,\\
    \loss_\text{col}^i(\ray) = \lvert\lvert \hat{C}_i(\ray) - C_i(\ray)\lvert\lvert \>,
    \label{eq:loss_col}
\end{gather}
%
where $C_i(\ray)$ is the observed color for pixel with ray $\ray$ in image $i$ and $\calR_i$ is the set of rays in frame $i$.


% In our case, we also need to estimate the camera pose with respect to the object. We thus also optimize on the camera pose in the object coordinate system by solving:
% %
% \begin{align}
%     \label{eq:complete_loss}
%     \theta^*, \{\campose_i^*\}_{i=1}^N &= \arg\min_{\theta, \{\campose_i\}_{i=1}^N} \sum_i \sum_{\ray\in \calH_i} \Big(\loss_\col^i(\ray)+\loss_\seg^i(\ray)\Big) \> .
% \end{align}
% %
% $\campose_i$ is the camera pose in the object coordinate system for frame $i$. $\calH_i$ is the set of object and background rays in frame $i$ and the direction and origin of ray $\ray\in\calH_i$ is a function of the camera pose $\campose_i$. Remember that we segment the object, hand and background using pre-trained networks~\cite{boerdijk2020learning,wu2021seqformer}. $\loss_\col^i$ is the photometric loss between rendered color $\hat{C}_i(\ray)$ and observed color $C_i(\ray)$, as defined in Eq.~\eqref{eq:loss_col} for frame $i$. We use only rays originating from the object and background pixels in Eq.~\eqref{eq:complete_loss} and ignore the hand pixels as the hand occludes the object during manipulation and the color of the object in the occluded regions is unknown.
\shreyas{
In our case, we also need to estimate the camera pose with respect to the object. We thus also optimize on the camera pose in the object coordinate system by solving:
%
\begin{align}
    \label{eq:complete_loss}
    \theta^*, \{\campose_i^*\}_{i=1}^N &= \arg\min_{\theta, \{\campose_i\}_{i=1}^N} \sum_i  \Big(\sum_{\ray\in \calH_i} \loss_\col^i(\ray)+ \sum_{\ray\in \calM_i} \loss_\seg^i(\ray)\Big) \> .
\end{align}
%
\shreyasrmk{will fix the eqn overflow}$\campose_i$ is the camera pose in the object coordinate system for frame $i$. $\calH_i$ is the set of object rays in frame $i$, $\calM_i$ is the set of object and background rays in images $i$ and the direction and origin of ray $\ray\in\{\calH_i, \calM_i\}$ is a function of the camera pose $\campose_i$. $\loss_\col^i$ is the photometric loss between rendered color $\hat{C}_i(\ray)$ and observed color $C_i(\ray)$, as defined in Eq.~\eqref{eq:loss_col} for frame $i$. We use only rays originating from the object or background pixels in Eq.~\eqref{eq:complete_loss} and ignore the hand pixels as the hand occludes the object during manipulation and the color of the object in the occluded regions is unknown.}

The second term $\loss_\seg(\ray)$ in Eq.~\eqref{eq:complete_loss} is a ``segmentation loss'' for ray $\ray$:
%
\begin{align}
    \label{eq:seg_loss}
    \loss_\seg^i(\ray) &= \BCE\Big(\max_k~\{o_\theta(\bx_k)\}, S_i(\ray) \Big) \> ,
\end{align}
%
where $\BCE(\cdot)$ is the binary cross-entropy loss, and $S_i(\ray)$ is the observed object segmentation value for ray $\ray$ in frame $i$. $S_i(\ray)$ is equal to 1 if the pixel corresponding to ray $\ray$ lies on the object according to the image segmentation, and 0 otherwise.  $\max_k~\{o_\theta(\bx_k)\}$ is the maximum occupancy along ray $\ray$, accroding to the estimated occupancy field $o_\theta(.)$. This maximum occupancy should also be equal to 1 if the ray intersects the object and to 0 otherwise.

We detail in the next section how we solve Eq.~\eqref{eq:complete_loss}.


==> 3old_background.tex <==
\section{Volumetric Rendering of an Implicit Surface}

\vincentrmk{I am not sure this is the right place.  Shouldnt we merge this with the Problem Formulation section, around Paragraph 2?}

%The implicit surface is estimated by first differentiably rendering the surface on to multiple views, followed by comparison with observed RGB images for photometric consistency. 

%by Oechsle et al. in 

% model the implicit surface and is a mapping given by,


\vincent{
We use an occupancy field to represent the surface of the object to be reconstructed. 
In this section, we provide an overview of the volumetric rendering scheme for occupancy fields which we use for reconstructing the object. This rendering scheme was proposed for UNISURF~\cite{unisurf} and estimates the object surface from multi-view posed images.
An occupancy field is represented by a deep network that implements a mapping of the form
%
\begin{equation}
    o_\theta(\bx): \mathbb{R}^3 \longrightarrow [0,1] \> ,  
\end{equation}
%
where $\theta$ represents the parameters of the network and $\bx$ the 3D coordinates of a point in the object coordinate system. The object surface $\calS$ is represented by the set of 3D points $\bx_\calS$ such that $o_\theta(\bx_\calS)=0.5$. A color field $c_\theta(\bx, \bd, \bn_\bx, \bh_\bx)$ is used to represent the color at each 3D point and is conditioned on the viewing ray direction $\bd$, the normal $\bn_\bx$ at point $\bx$ and the geometry feature $\bh_\bx$ at point $\bx$. 


Such a model accounts for the specular reflections on the object surface under the Phong reflection model~\cite{HughesDamEtAl13} when the position of the light source w.r.t to the object is fixed. The static pose between the object and the light source in all the images results in a constant incoming light radiance at any point on the object surface as shown in Figure~\ref{fig:static_object}.
\vincentrmk{add a ref to our problem}


The rendered color at a pixel is obtained by integrating the color values along the ray $\ray$ originating from the camera center and passing through the pixel. The continuous integration is approximated using quadrature and is given by
%
\begin{gather}
    \hat{C}_i(\ray) = \sum_{k=1}^M \gamma(\bx_k) c_\theta(\bx_k, \bd, \bh_{\bx_k}, \bn_{\bx_k}) \>, \\
    \gamma(\bx_k) = o_\theta(\bx_k)\prod_{l<k}\big(1-o_\theta(\bx_l)\big) \nonumber \> ,
    \label{eq:rend_unisurf}
\end{gather}
%
where $\{\bx_k\}$ are $M$ samples along the ray $\ray$, $\hat{C}_i(\ray)$ represents the rendered colored in frame $i$ at pixel $\ray$, and $\gamma(\bx_k)$ is the alpha-blending coefficient that evaluates to 1 if point $\bx_k$ is on the surface of the object and 0 otherwise.

In UNISURF, the network parameters are obtained by minimizing the photometric loss given by
%
\begin{gather}
    \theta^* = \arg\min_\theta \sum_i \sum_{\ray \in \calR_i} \loss_{\text{col}}^i(\ray) \nonumber \> ,\\
    \loss_\text{col}^i(\ray) = \lvert\lvert \hat{C}_i(\ray) - C_i(\ray)\lvert\lvert \>,
    \label{eq:loss_col}
\end{gather}
%
where $C_i(\ray)$ is the observed color for pixel with ray $\ray$ in image $i$ and $\calR_i$ is the set of rays in frame $i$.
}


==> 4old_formulation.tex <==
\textvars{col,seg,BCE,opf,reg,inc,trac,OF,dep}

\section{Problem Formulation}
\label{sec:problem}

\shreyas{
Our setup for in-hand object scanning consists of a static RGB camera and an unknown rigid object being handled by one or two hands for in the field of view of the camera for scanning. We assume a static background whose image is either obtained separately or is estimated from the sequence using the segmentation masks of the hand and the  object. We use a pre-trained network from \cite{boerdijk2020learning} to segment the dynamic foreground and combine it with accurate hand segmentations obtained from \cite{wu2021seqformer} to obtain the masks of the hand, the object, and the background.


% \vincentrmk{I understand what you mean but this can be a bit confusing. Do we need it? :}\shreyasrmk{The other way is to describe everything in the camera coordinate system (right now all the equations are in object coordinate system). I think people are used to seeing nerf rendering equations in the object coordinates and changing this to camera coordinates may make them look complex? Fig.2 is great, how about I refine it a little bit and refer to it for this interpretation?} \vincentrmk{Sure, do not hesitate to change it}

We represent the object surface using the occupancy field and color field similar to UNISURF~\cite{unisurf}. However, the varying position of the object w.r.t the light source results in varying incoming light radiance, $\omega_i$ on the object surface as illustrated in Figure~\ref{fig:static_camera} for the in-hand object scanning setup. Under the Phong reflection model~\cite{HughesDamEtAl13}, the observed radiance at a point on the object surface depends on the viewing direction, $\bd$, direction of the normal at the point, $\bn$ and the incoming light direction, $\omega_i$. As the relative position between the camera and the light source remains fixed, the incoming light direction can be parameterized as $\omega_i = f(\bx, \bd, \bn, p)$, where $p$ is the length of the viewing ray. $p$ is computed as the distance between the camera optic center and the 3D point at which the observed radiance is calculated. Thus, we represent the color field as $c_\theta(\bx,\bd, p,\bn_x,\bh_x)$ where we additionally condition the color field on viewing ray length compared to previous approaches~\cite{unisurf,Mildenhall2020nerf,idr}.

% Similarly to UNISURF~\cite{unisurf}, we represent the object to reconstruct by an occupancy field network and a color field network at every 3D point in the object coordinate system and aim to find the optimal parameters for these two networks. 
% There is however a very important difference: Standard NeRF methods~\cite{nerf, unisurf, other_nerf_papers} work under the assumption of a static scene and light environment as shown in Figure~\ref{fig:static_object},  i.e, the relative pose between the object and the light source is fixed and only the relative pose between the object and the camera changes in each frame. This allows these methods to condition the observed radiance at any 3D point on the surface only on the viewing ray direction and the surface normal direction at that point defined in the object coordinate system to capture the non-Lambertian effects. 

% \shreyas{In our case, as illustrated in Figure~\ref{fig:static_camera}, the relative pose between the object and light source also changes in addition to camera-object pose. As a result, the observed radiance on the object surface which is a function of the incident light direction and the viewing direction, depends on the object-camera relative pose, camera-light relative pose and the surface normal. As the camera-light relative pose is fixed in all the images this dependency can be factored out. Hence, we model the observed radiance along each viewing ray as a function of surface normal, ray direction and ray \emph{length} to capture the non-Lambertian effects.}
% In our case, as the camera and the light sources with their relative poses fixed capture the static object from different views, we also need to condition the color field on the ray \emph{length}.
% \vincentrmk{Isnt this because the rays are defined in the camera coordinate system?  What happens if you consider rays in the object coordinate system?  We should probably discuss the alternatives.}\shreyasrmk{I think its independent of what coordinate system we use. The color depends on incident light direction, view direction and normal. Incident light direction always changes in our case unlike standard-Nerf and hence the need to model the color based camera-object-light relative poses. The fact that camera-light poses is fixed allows us to only consider camera-object pose. An interesting point is that if we consider directional light instead of point light source, then we can do away with the dependency on ray length and it becomes standard-nerf modelling again!}

%Similar to \cite{unisurf}, we represent the object to be reconstructed by an occupancy field network $o_\theta(\bx)$ and the color field network $c_\theta(\bx)$ at every 3D point, $\bx$, and aim to find the optimal network parameters $\theta$. Traditional NeRF methods~\cite{nerf, unisurf, other_nerf_papers} that work under the assumption of static scene and light setup, but varying camera locations condition the color field on the viewing direction, $\bd$ to model non-Lambertian surfaces. In our case, as the camera and the light sources with their relative poses fixed capture the static object from different views, we model the color field also conditioned on the ray length. 

% This is illustrated in Figure~\ref{fig:raydist}: When a 3D point on the object surface is viewed by the camera under two different object poses, its color may change even if the direction of the line of sight remains the same. This is because the angle between the line of sight and the light direction changes, and the amount of light reflected toward the camera is a function of this angle. A simple way to capture this phenomenon is to condition the color field on the distance between the camera and the 3D point.

% \vincentrmk{this does not capture everything, no?  The color also depends on the normal. If the object rotates around the point, the ray direction and length and light direction do not change but the normal changes, which will change the point's color.  Maybe it does not matter because it does not happen in practice? }\shreyasrmk{Yes, color depends on normal also. But normal is not explicitly calculated (but some works do) and the color is a function of the feature embedding at a 3D point and the view  direction. The feature embedding represents the normal.}

% shows an example of a point on the object surface viewed by a camera at two different poses of the object relative to the camera such that the viewing direction is the same. A point-light source located at a fixed position, $\calM$ w.r.t to the camera results in two different incident light directions and is a function of viewing direction, ray length and camera position $\calM$. Our color field $c_\theta(\bx,\bd,p)$ is thus conditioned on view direction, $\bd$ and ray length, $p$ as $\calM$ is constant in all the images. \vincentrmk{Maybe $c$ should be bold since it is a (color) vector?}

% \begin{figure}
%     \centering
%     \includegraphics[trim=100 180 400 100, clip, ,width=1\linewidth]{figures/method/ray_dist.pdf}
%     \caption{Incident and reflected rays under two different poses of the object relative to the camera. The relative position between the camera and the point-light does not change during the capture. The observed object color is  dependent both on the viewing ray direction and the ray length as the object changes its pose while the camera and the light source remain static.}
%     \label{fig:raydist}
% \end{figure}


\begin{figure}
    \centering
    \begin{minipage}{1\linewidth}
        \subcaptionbox{Static-object and static-light capture setup\label{fig:static_object}}
        {\includegraphics[page=1,width=1\linewidth,trim=140 150 75 80, clip,]{figures/method/ray_length.pdf}}
    \end{minipage}
    \begin{minipage}{1\linewidth}
        \subcaptionbox{Static-camera and static-light capture (In-hand scanning) setup \label{fig:static_camera}}
        {\includegraphics[page=2,width=1\linewidth,trim=130 150 105 120, clip,]{figures/method/ray_length.pdf}}
    \end{minipage}
    \caption{\shreyas{(a) In the case of the standard NeRF setting, the camera moves with respect to the object, and the observed radiance at a 3D point depends only on the viewing ray direction and the normal as the incident light direction is fixed in all frames. (b) In the case of in-hand scanning, the object moves with respect to the fixed camera and the lights setup, and the incident light direction at a 3D point on the surface of the object depends on the camera-object relative pose. To capture this, we simply condition the radiance on the distance between the camera and the point (ray length), in addition to the direction of the viewing ray and normal.}}
    \label{fig:raydist}
\end{figure}

A second major difference with other NeRF approaches is that we need to estimate the camera pose with respect to the object, while previous approaches often assume the camera poses to be given. We thus estimate the object's shape and appearance by solving:
%
\begin{align}
    \label{eq:complete_loss}
    \theta^*, \{\campose_i^*\}_{i=1}^N &= \arg\min_{\theta, \{\campose_i\}_{i=1}^N} \sum_i \sum_{\ray\in \calH_i} \Big(\loss_\col^i(\ray)+\loss_\seg^i(\ray)\Big) \> .
\end{align}
%
$\campose_i$ is the camera pose in the object coordinate system for frame $i$. $\calH_i$ is the set of object and background rays in frame $i$ and the direction and origin of ray $\ray\in\calH_i$ is a function of the camera pose $\campose_i$. Remember that we segment the object, hand and background using pre-trained networks~\cite{boerdijk2020learning,wu2021seqformer}. $\loss_\col^i$ is the photometric loss between rendered color $\hat{C}_i(\ray)$ and observed color, $C_i(\ray)$ as defined in Eq.~(\ref{eq:loss_col}) for frame $i$. $\loss_\seg$ is the segmentation loss which we explain later.

Unlike the static-object based setup as in Figure~\ref{fig:static_object}, the background in the in-hand object scanning setup is static as in Figure~\ref{fig:static_camera} whose image is assumed to be available in this paper. We thus modify the rendering equation in Eq.~(\ref{eq:rend_unisurf}) to include pixels from the background image as below,
%
\begin{align*}
    \hat{C}_i(\ray) &= \sum_{k=1}^M \gamma(\bx_k) c_\theta(\bx_k,\bd, p_k, \bn_{\bx_k}, \bh_{\bx_k}) + \gamma_{bg}c_{bg}(\ray) \> ,
\end{align*}
%
where the $M$ samples $\{\bx_k\}$ along the ray $\ray$ are in the object coordinate system and the blending coefficients $\gamma(\bx_k)$ is as defined in Eq.~(\ref{eq:rend_unisurf}). The blending coefficient for the background pixel is computed as $\gamma_{bg} = \prod_{k}\big(1-o_\theta(\bx_k)\big)$. $c_{bg}(\ray)$ is the background pixel value at pixe $\ray$. When the object masks are accurate, the background pixels in each image can be set to black color and original rendering equation in Eq.~(\ref{eq:rend_unisurf}) can be used. However, since the masks obtained from the segmentation network~\cite{boerdijk2020learning} are often noisy we use background pixels during rendering to mitigate the effect of inaccurate masks. 

We use only rays originating from the object and background pixels in Eq.~(\ref{eq:complete_loss}) and ignore the hand pixels as the hand occludes the object during manipulation and the color of the object in the occluded regions is unknown.

% For $\hat{C}(\ray)$, we follow the rendering equation of UNISURF:
% %
% \begin{align}
% \label{eqn:rend_eqn}
%     \hat{C}(\ray) &= \sum_{k=1}^M \gamma(\bx_k) c_\theta(\bx_k,\bd,p_k) + \gamma_{bg}c_{bg}(\ray)\> .
% \end{align}
% %
% $c_\theta(\bx_k,\bd,p_k)$ is the neural color field for point $\bx_k$ defined in the object coordinate system (see Figure~\ref{fig:static_camera}) sampled at $M$ points along the ray $\ray\in\calR_i$ whose direction is $\bd$. $p_k$ is the ray length and is the distance between $\bx_k$ and the camera center for frame $i$. The 3D point $\bx_k$ and direction $\bd$ are expressed in the object coordinate system. $c_{bg}(\ray)$ is the color of the static background image that is pre-computed or readily available. $\gamma(\bx_k)$ and $\gamma_{bg}$ are the blending coefficients for the color values computed on the ray $\ray$ and is computed as
% %
% \begin{align}
% \label{eqn:gamma}
%     \gamma(\bx_k) &= o_\theta(\bx_k) \prod_{l<k} \big(1-o_\theta(\bx_l)\big) \> ,\\
%     \gamma_{bg} &= \prod_{k=1}^M \big(1-o_\theta(\bx_l)\big) \> ,
% \end{align}
% %
% \vincentrmk{do gamma and $o$ really depend on the camera pose?}\shreyasrmk{No, $\gamma$ and $o$ are computed on points in the object coordinate system, so they are independent of camera pose.}
% where $o_\theta(\bx_k)$ is the neural occupancy field computed at point $\bx_k$.

The second term $\loss_\seg(\ray)$ in Eq.~\eqref{eq:complete_loss} is a ``segmentation loss'' for ray $\ray$:
%
\begin{align}
    \label{eq:seg_loss}
    \loss_\seg^i(\ray) &= \BCE\Big(\max_k~\{o_\theta(\bx_k)\}, S_i(\ray) \Big) \> ,
\end{align}
%
where $\BCE(\cdot)$ is the binary cross-entropy loss, and $S_i(\ray)$ is the observed object segmentation value for ray $\ray$ in frame $i$. $S_i(\ray)$ is equal to 1 if the ray projects on the object segmentation, and 0 otherwise.  $\max_k~\{o_\theta(\bx_k)\}$ is the maximum occupancy along ray $\ray$, which should also be equal to 1 if the ray intersects the object and to 0 otherwise.

We detail in the next section how we solve Eq.~\eqref{eq:complete_loss}.
}

% and $\loss_\text{seg}(\ray)$ is a segmentation loss for the ray $\ray$ respectively, $C(\ray)$ is the observed color of ray $\ray$, $\calR$ is the set of all pixels in all the frames, $BCE(\cdot)$ is the binary cross-entropy loss, and $S_o(\ray)$ is the observed object segmentation value for the ray $\ray$. We drop the dependency of $\hat{C}$ on the pose, $\campose$ for brevity.

% We drop the dependency of $\hat{C}$ on the pose, $\campose$ for brevity.

% We follow the rendering equation described in UNISURF~\cite{unisurf} to perform volumetric rendering with $M$ 3D points $\{\bx_{k,i}\}_i$ sampled along the ray, $\ray_k=\bo(\campose_k)+t\bd(\campose_k)$ originating from the camera $k$ whose pose is $\campose_k$, camera center is $\bo(\campose_k)$ and the ray direction is $\bd(\campose_k)$. The coordinates $\bx_i^k$, ray direction $\bd$ and ray length, $p_i = \|\bx_i^k-\bo(\campose_k)\|_2$ are encoded using the sinusoidal representation~\cite{unisurf} and the rendering equation is given by
% %
% \begin{align}
% \label{eqn:rend_eqn}
%     \hat{C}(\ray_k;\campose_k) &= \sum_{i=1}^M \gamma(\bx_{k,i};\campose_k) ~c_\theta(\bx_{k,i},\bd,p_i;\campose_k),\\
%     \gamma(\bx_{k,i};\campose_k) &= o_\theta(\bx_{k,i};\campose_k) \prod_{j<i} \big(1-o_\theta(\bx_{k,i};\campose_k)\big)
% \end{align}
% %
% where $\hat{C}$ is the rendered pixel value. The parameters $\theta^*$ representing the object and the camera poses $\{\campose_i^*\}_{i=1}^N$ is given by
% %
% \begin{align}
%     \label{eq:first_loss}
%     \theta^*, \{\campose_i^*\}_{i=1}^N &= \arg\min_{\theta, \{\campose_i\}_{i=1}^N} \sum_{\ray\in \calR} \Big(\loss_\text{col}(\ray)+\loss_\text{seg}(\ray)\Big) \\
%     \loss_\text{col}(\ray) &= \|\hat{C}(\ray) - C(\ray)\|_2\nonumber \\
%     \loss_\text{seg}(\ray) &= BCE\Big(\max_i~\{o_\theta(\bx_{k,i})\}, S_o(\ray) \Big) \nonumber,
% \end{align}
% %
% where $\loss_\text{col}(\ray)$ and $\loss_\text{seg}(\ray)$ are the RGB color loss and segmentation loss for the ray $\ray$ respectively, $C(\ray)$ is the observed color of ray $\ray$, $\calR$ is the set of all pixels in all the frames, $BCE(\cdot)$ is the binary cross-entropy loss, and $S_o(\ray)$ is the observed object segmentation value for the ray $\ray$. We drop the dependency of $\hat{C}$ on the pose, $\campose$ for brevity.




%We follow the rendering equation described in UNISURF~\cite{unisurf} to perform volumetric rendering with $M$ 3D points $\{\bx_{k,i}\}_i$ sampled along the ray, $\ray_k=\bo(\campose_k)+t\bd(\campose_k)$ originating from the camera $k$ whose pose is $\campose_k$, camera center is $\bo(\campose_k)$ and the ray direction is $\bd(\campose_k)$. The coordinates $\bx_i^k$, ray direction $\bd$ and ray length, $p_i = \|\bx_i^k-\bo(\campose_k)\|_2$ are encoded using the sinusoidal representation~\cite{unisurf} and the rendering equation is given by
% %
% \begin{align}
% \label{eqn:rend_eqn}
%     \hat{C}(\ray_k;\campose_k) &= \sum_{i=1}^M \gamma(\bx_{k,i};\campose_k) ~c_\theta(\bx_{k,i},\bd,p_i;\campose_k),\\
%     \gamma(\bx_{k,i};\campose_k) &= o_\theta(\bx_{k,i};\campose_k) \prod_{j<i} \big(1-o_\theta(\bx_{k,i};\campose_k)\big)
% \end{align}
% %
% where $\hat{C}$ is the rendered pixel value. The parameters $\theta^*$ representing the object and the camera poses $\{\campose_i^*\}_{i=1}^N$ is given by
% %
% \begin{align}
%     \label{eq:first_loss}
%     \theta^*, \{\campose_i^*\}_{i=1}^N &= \arg\min_{\theta, \{\campose_i\}_{i=1}^N} \sum_{\ray\in \calR} \Big(\loss_\text{col}(\ray)+\loss_\text{seg}(\ray)\Big) \\
%     \loss_\text{col}(\ray) &= \|\hat{C}(\ray) - C(\ray)\|_2\nonumber \\
%     \loss_\text{seg}(\ray) &= BCE\Big(\max_i~\{o_\theta(\bx_{k,i})\}, S_o(\ray) \Big) \nonumber,
% \end{align}
% %
% where $\loss_\text{col}(\ray)$ and $\loss_\text{seg}(\ray)$ are the RGB color loss and segmentation loss for the ray $\ray$ respectively, $C(\ray)$ is the observed color of ray $\ray$, $\calR$ is the set of all pixels in all the frames, $BCE(\cdot)$ is the binary cross-entropy loss, and $S_o(\ray)$ is the observed object segmentation value for the ray $\ray$. We drop the dependency of $\hat{C}$ on the pose, $\campose$ for brevity.

==> 5old_method_v1.tex <==




\section{The proposed method}



Optimizing directly Eq.~\eqref{eq:complete_loss} is prone to fail: As we show in the experiment section, a random (or fixed) initialization of the pose parameters followed by an optimization similar to the one in BARF~\cite{barf} leads to degenerate solutions. We therefore obtain estimates of poses using frame-to-frame tracking and incremental object reconstruction. The estimated poses are refined using the global optimization in Eq.~\eqref{eq:complete_loss} which considers all the frames in the sequence.

% Figure~\ref{fig:pipeline} shows our pipeline for object reconstruction and pose estimation from the input RGB sequence. 
Simultaneous 3D pose tracking and reconstruction is  prone to drift, and during our early experiments, we noticed this happens very often on in-hand object tracking sequences such as the ones from the HO-3D dataset~\cite{hampali-cvpr20-honnotate}: While the object rotates, there can be a drastic disappearance of visual features followed by the emergence of new visual features that are not reconstructed yet, as illustrated in Figure~\ref{fig:pipeline} on the left. We observed these situations quickly result in important drift. \vincentrmk{we probably need to show that in the experiments}
As shown in Figure~\ref{fig:pipeline} our solution is to first split the input sequence into overlapping video segments on which we perform tracking independently to obtain a first estimate of the camera poses, before merging the estimates for the segments and running a global optimization. To split the sequence, we introduce a heuristics based on the apparent area of the object, as drift is likely to occur when the object becomes smaller in the image. 

\vincentrmk{i will add more details about the other steps}

Section~\ref{sec:splitting} details how we split the sequence. We then explain how we perform simultaneous pose tracking and reconstruction on each segment in Section~\ref{sec:segment_tracking} to obtain a first estimate of the poses. Section~\ref{sec:stitch} explains how we perform the global optimization of Eq.~\eqref{eq:complete_loss} using the estimated poses.



% As the object undergoes a large motion in 3D during scanning, solving Eq.~\eqref{eq:full_loss} requires coarse initialization of the camera poses: As we show later in our experiments, random or fixed initialization of the pose parameters followed by optimization similar to BARF~\cite{barf} leads to degenerate solutions. Though COLMAP~\cite{colmap} is the standard method for obtaining coarse level pose estimates in NeRF-based methods~\cite{nerf,nerf_w,nerv,nerd}, it fails to obtain sufficient keypoint matches that are necessary for pose estimation in the regions of the object that contain less texture. As a result, COLMAP can provide reliable pose initialization only for highly-textured objects. 

% Our approach to reconstruction of generic objects (both textured and non-textured) and their pose estimation is based on tracking, which incrementally reconstructs the object surface while simultaneously optimizing the poses at each tracking step. As tracking algorithms suffer from drift~\cite{}, we divide the video sequence into multiple overlapping segments and reconstruct parts of the object surface and obtain pose estimates within each segment independently. Finally, using the camera poses obtained in each segment, the segments are \textit{stitched} together and a global optimization similar to Eq.~\eqref{eq:first_loss} is performed to achieve complete object reconstruction. We provide details about the intra-segment tracking, inter-segment optimization and the algorithm for dividing the video sequence into multiple segments below.


% I moved the splitting at the beginning because I think it is important and also gives an intuition about the video segments

\begin{figure}
    \centering
    \includegraphics[trim=90 130 90 2, clip, width=1\linewidth]{figures/method/seg_area.pdf}
    \caption{Segmenting the input video into easy-to-track segments. We plot the object segmentation area obtained by segmenting the background and the hand over time. We use the local maxima and minima of this plot as segment boundaries. Note that we can track ``backward'' in time, from a local maximum to a local minimum.}
    \label{fig:seg_area}
\end{figure}


\subsection{Segmenting the video sequence}

We split the input sequence into segments so that tracking on each segment is unlikely to drift much.  
We privilege segments in which the object surface self-occludes with time, rather than segments in which new surface portions appear as this is likely to provoke drift.  This is however \emph{a priori} a chicken-and-egg problem, as we do not know the surface yet. Fortunately, we can consider the area of the 2D object's silhouette, which we can obtain from the pre-trained segmentation networks~\cite{boerdijk2020learning,wu2021seqformer}\vincentrmk{why 2 references?}. \vincent{As illustrated in Figure~\ref{fig:seg_area}, we divide the sequence into multiple segments such that each segment starts at a frame where the object segmentation area reaches a local maximum, and ends at a frame where the object area reaches a local minimum. Figure~\ref{fig:seg_area} shows the plot of object segmentation and the three segments. The direction of tracking within the segment can be in the reverse direction of capture, as the full video is taken as input. Disappearance of object surfaces due to self-occlusion and emergence of new object surfaces during in-hand object scanning indeed correspond to local minima in the apparent 2D surface of the object as we show with a formal proof in the supplementary material\vincentrmk{really?  It probably would not happen in practice but cant you make the object getting closer to the camera while rotating it to make this heuristic fails?  We probably should add this is under the assumption the distance of the object to the camera remains about constant.}. Thus, by stopping tracking at the end of the segments which are local minimum in the object area we avoid large drifts.}

% We therefore start segments at frames where this area reaches a local maximum. Since we have access to the full sequence, we create in general two segments starting from the same local maximum, one continuing toward the ``future'' of the local maximum, the second one continuing toward the ``past''.


A second advantage of this strategy is that the object's surface in the frames corresponding to local maxima of the object's area tend to be nearly parallel to the image plane. We also refer the reader to the supplementary material for proof. We exploit this property to converge better to the correct surface by introducing a regularization term that encourages nearly parallel surface in the first frame of each segment. 

The neighboring segments overlap by at least one frame, which we used to merge the estimated pose trajectories before running a global optimization of Eq.~\eqref{eq:full_loss}.




% We extend the segments by one frame at the two extremities so that to consecutive segments overlap for 3 frames\vincentrmk{correct?}. This allows us to merge the estimated surfaces and camera trajectories in a consistent way, before running a global optimization of Eq.~\eqref{eq:full_loss}.

% Our choice of the algorithm for dividing the video sequence into multiple segments is driven by our tracking procedure explained in Section~\ref{sec:tracking_method} and to obtain accurate tracking within each segment. Recall that the regularization term in Eq.~\eqref{eq:reg_loss} enforces near-plane surface reconstruction in the tracking step, $t=0$. We divide the video sequence into multiple segments and determine the tracking direction in each segment such that the observed object surface in the first frame of the segment is nearly-parallel to the image plane. We rely on object reprojection area in the image to determine the segment boundaries in the sequence and the tracking direction within the segment.


% More specifically, frames with large object reprojection area contain object surfaces that are nearly-parallel to the image plane (see supplementary material for formal proof\vincentrmk{that's cool :)}) and are thus good starting points for tracking. Figure~\ref{fig:seg_area} shows the plot of the object reprojection area through the sequence and sampled frames. The local maxima of the reprojection area are representative of the frames with large parallel object surface and are thus the segment-start boundaries. The local minima are chosen to be the segment-end boundaries as these are representative of the frames where the tracked object surface in the segment begins to self-occlude (see Figure~\ref{fig:seg_area}). We also set a threshold on the segment length to discard noisy segment boundaries and enforce 1-2 frame overlap between the segments.



\begin{figure}
    \centering
    \includegraphics[trim=10 160 10 100, clip, width=1\linewidth]{figures/reg_term/reg_wt.pdf}
    \caption{Ground-truth object mesh and pose, w/o regularization term, w/ regularization term.}
    \label{fig:my_label}
\end{figure}

% \begin{figure*}
%     \begin{minipage}{.19\linewidth}
%     \centering
%     \subcaptionbox{Single Frame Real Depth}
%     {\includegraphics[page=1,trim=140 105 170 40, clip, width=1\linewidth]{figures/reg_term/reg_term2.pdf}}~\vrule~%
%     \subcaptionbox{Single Frame w/o Reg.\label{fig:1frame_wo_reg}}
%     {\includegraphics[page=2,trim=140 105 170 40, clip, width=1\linewidth]{figures/reg_term/reg_term2.pdf}}~%
%     \subcaptionbox{Five Frames w/o Reg.\label{fig:5frames_wo_reg}}
%     {\includegraphics[page=3,trim=140 105 170 40, clip, width=1\linewidth]{figures/reg_term/reg_term2.pdf}}~%
%     \subcaptionbox{Single Frame w/ Reg.\label{fig:1frame_w_reg}}
%     {\includegraphics[page=4,trim=140 105 170 40, clip, width=1\linewidth]{figures/reg_term/reg_term2.pdf}}~%
%     \subcaptionbox{Five Frames w/ Reg.\label{fig:1frame_w_reg}}
%     {\includegraphics[page=5,trim=140 105 170 40, clip, width=1\linewidth]{figures/reg_term/reg_term2.pdf}}
%     \end{minipage}
%     % \vspace{-0.5cm}
%     \caption{Importance of regularization Term $\loss_\text{reg}$. Top view of (a) the camera and the point cloud of the object captured by a depth camera (used only for visualization), and (b-e) the occupancy field retrieved  our method under different settings. The images of the point cloud and the different occupancy field rendered from the point of view of the camera are shown in the insets. While these images are very similar, they correspond to 3D shapes that can be very different: The occupancy field obtained without our regularization term with one or five frames is distorted (b and c), more so in the low-texture regions of the object (see bottom part of the $\textit{power\_drill}$). When using the regularization term with a single frame (d), the occupancy field is mostly constrained to a plane parallel to the image plane (shown in green). With multiple frames and the regularization term (e), we obtain more accurate reconstruction of the object surface. }
%     \label{fig:reg_term}
%     \vspace{-0.3cm}
% \end{figure*}

% \subsection{Simultaneous reconstruction and pose estimation within segments}
\subsection{Per-segment optimization}
\label{sec:tracking_method}

We now explain how we retrieve a first estimate of parameters $\theta$ of the occupancy and color fields and of poses $\calT_j$ for the frames of a video segment.

\vincent{
Let's denote the frames in the segment by $\{\calS_i\}_{i=0}^T$. We successively minimize, for t in $[0;T]$:
%
\begin{align}
\label{eq:inc_loss}
    \sum_{i=0}^t \sum_{\ray\in\calR(\calS_i)} \loss_\col^i(\ray) + \loss_\seg^i(\ray) &+ \loss_\opf^i(\ray) + \loss_\reg^i(\ray) \;+ \nonumber \\& \sum_{i=0}^{t-1}\sum_{\ray\in\calR(\calS_i)}\loss_\dep^i(\ray) \> ,
\end{align}
%
over $\theta$ and the $\{\calT_i\}_{i=1}^t$ poses. The first two terms $\loss_\col$ and $\loss_\seg$ are the color and segmentation losses as defined in Eq.~\eqref{eq:complete_loss}. $\loss_\opf$ is a loss based on optical flow that provides constraints on the poses, $\loss_\reg$ is a regularization term that prevents degenerate object shapes, and $\loss_\dep$ is a depth loss using rendered depths that stabilizes the tracking. At each tracking step, $\loss_\dep$ is only applied to previously tracked frames using the depth map that is rendered and stored for each frame after it is tracked. We provide more details about the latter three loss terms later in this section.

The network parameters $\theta$ are initialized from their estimate after the previous tracking step $t-1$. %Optimizing over all frames from 0 to $t$ avoids forgetting the object surface reconstructed in the previous views $\{\calS_i\}_{i=0}^{t-1}$. 
% Recall that $\calT_i$ is the pose of the camera in the object coordinate system at frame $i$. 
The camera pose $\calT_t$ for $t>1$ is initialized using the second-order motion model applied to previous poses $\{\calT_i\}_{i=0}^{t-1}$. Camera pose $\calT_0$ is initialized to a fixed distance from the origin of the object coordinate system and in a direction such that the imaging plane faces the origin. 

% $\calT_0$ is fixed to the identity, and $\calT_1$ is initialized to the identity\vincentrmk{ok it shouldnt be the identity, i need to fix that}. Fixing $\calT_0$ is required as the object surface and the camera trajectory are defined up to a rigid motion. This also fixes the object coordinate system, and the 3D points we sample along the rays are defined in this coordinate system.
}

% of the cameras corresponding to frames in $\calS_t$ are initialized using the second-order motion model on the trajectory of the poses of $\{\calS_i\}_{i=0}^{t-1}$.


% Let $\calS_t$ denote the set of new frames from the sequence that are added at tracking step $t$. $\{\calS_i\}_{i=0}^{t-1}$ denotes the set of frames \vincentrmk{If $\calS_i$ is a set of frames, this is a set of set of frames} which are used for tracking in the previous $t-1$ steps. The poses of the cameras corresponding to frames in $\calS_t$ are initialized using the second-order motion model on the trajectory of the poses of $\{\calS_i\}_{i=0}^{t-1}$. The occupancy and color network parameters, $\theta$, at step $t$ are initialized from the previous tracking step $t-1$. 


% Further, after each tracking step $t$, we render and store the set of depth maps, $\calD_t$ in the views $\calS_t$ using the optimized poses. \vincentrmk{What do you use them for?}

% The optimization at each tracking step is intended to update the network parameters, $\theta$, such that:
% %
% \begin{itemize}
%     \item the updated parameters also represent the incremental new surface visible in views $\calS_t$.
%     \item the object surface reconstructed in the previous views $\{\calS_i\}_{i=0}^{t-1}$ is intact and not \textit{forgotten}
% \end{itemize}
% %
% The incremental surface visible in $\calS_t$ is reconstructed by minimizing the objective function
% %
% \begin{equation}
% \label{eq:inc_loss}
%     \loss_\inc = \sum_{i=0}^t \sum_{\ray\in\calR(\calS_i)} \loss_\col(\ray) + \loss_\seg(\ray) + \loss_\opf(\ray) + \loss_\reg(\ray) \> ,
% \end{equation}
% %
% where the former two terms $\loss_\col$ and $\loss_\seg$ are color and segmentation losses as defined in Eq.~\eqref{eq:first_loss}. $\loss_\opf$ is a loss based on optical flow and $\loss_\reg$ is a regularization term.
% We provide more details about the latter two terms below.


We now provide details about the loss terms we introduced in Eq.~\eqref{eq:inc_loss}.

\paragraph{Optical flow loss $\loss_\text{opf}^i$.}

This term provides additional constraints on the camera poses and is defined as
%
\begin{align}
    \loss_\opf^i(\ray) = \sum_k \gamma(\bx_k) \big(\pi_i(\bx_k) - \pi_{i-1}(\bx_k)  - \OF_{i-1}(\pi_{i-1}(\bx_k)) \big) \> ,
\end{align}
%
where the $\{\bx_k\}_i$ are 3D points along ray $\ray$. $\pi_i(\bx)$ is the 2D reprojection of point $\bx$ in camera frame $i$. $\OF_{i-1}$ is the optical flow between frame $i-1$ and frame $i$. In practice, we use \vincentrmk{..} method to estimate the flow. 


% This term provides additional constraints on the camera poses and is defined as
% %
% \begin{align}
%     \loss_\opf(\ray_k) = \sum_i &\Big(\pi\big( \campose_{\calN(k)}  \bx_{k,i}\big) - \pi\big( \campose_k  \bx_{k,i}\big) - OF_{\ray_k}\Big) \cdot \nonumber \\ 
%     &\gamma(\bx_{k,i};\campose_k), \nonumber
% \end{align}
% %
% where $\ray_k$ is the ray from the $k^\text{th}$ frame, $\{\bx_{k,i}\}_i$ are the samples along the ray $\ray_k$, $\campose_{\calN(k)}$ is the pose of the frame that is neighboring the frame $k$ with pose $\campose_k$, $\pi(\cdot)$ is the camera projection function, and $OF_{\ray_k}$ is the optical flow precomputed at pixel/ray $\ray_k$.

\shreyas{
\paragraph{Regularization term $\loss_\reg^i$.} During the first tracking steps (\ie, when $t$ is small), the occupancy field is under-constrained and needs to be regularized to avoid degenerate object shapes. We introduce a regularizer term that encourages reconstruction near the origin of the object coordinate system. It is defined as:
%
\begin{equation}
\label{eq:reg_loss}
    \loss_\reg^i(\ray) = \sum_k o_\theta(\bx_k) \exp{(\alpha \cdot \|\bx_k\|_2)} \> ,
\end{equation}
%
where $\alpha$ is a hyperparameter. Additionally, at $t=0$, $\loss_\reg^i$ results in a object surface that is parallel to the image plane. This can be proven by considering an orthographic projection of the rays and noting that for each ray $\ray$, $\loss_\reg(\ray)$ is minimized when $\|\bx_k\|$ is minimized, \ie, when $\bx_k$ is on a plane perpendicular to the ray direction and passing through the origin. We exploit this parallel plane property of the regularizer by choosing the first frame of the segment such that the observed object surface is nearly parallel to the image plane as mentioned in Section~\ref{sec:split}. Figure~\ref{fig:} shows the reconstructed surfaces with and without the regularizer term for an example. 
}

% Minimizing Eq.~\eqref{eq:inc_loss} is still underconstrained for small values of $t$ and results in degenerate solutions as shown by the occupancy fields in Figures~\ref{fig:1frame_wo_reg} and \ref{fig:5frames_wo_reg}. The distortion mainly occurs in low-texture regions, such as the bottom of the $\textit{power\_drill}$ object in Figure~\ref{fig:reg_term} where $\loss_\col$ cannot provide meaningful gradients to optimize the poses, while the rendered images are still reasonable. 

% We introduce a regularizer on the occupancy field to avoid degenerate solutions. This regularizer can be defined as
% %
% \begin{equation}
% \label{eq:reg_loss}
%     \loss_\reg^i(\ray) = \sum_k o_\theta(\bx_k) \exp{(\alpha \cdot \|\bx_k\|_2)} \> ,
% \end{equation}
% %
% where $\alpha$ is a hyperparameter. 

% This regularizer ensures that the object is reconstructed near the origin of the coordinate system and discourages artifacts in the occupancy field. It also encourages the reconstruction of surfaces that are nearly parallel to the image plane.  \vincentrmk{is it really a good thing? Should we emphasize this?}

% Moreover, when considering rays from a single camera located at a certain distance from the origin and pointing towards the origin, $\loss_\reg$ forces reconstruction of the object surface on a plane that is nearly parallel to the image plane and passing through the origin as shown in Figure~\ref{fig:1frame_w_reg}. 

% This can be proven by considering an orthographic projection of the rays and noting that for each ray $\ray$, $o_\theta(\bx_k) \in \{0,1\}$~\cite{unisurf} and $\loss_\reg(\ray)$ is minimized when $\|\bx_k\|$ is minimized, which is a point on a plane perpendicular to the ray direction and passing through the origin. When minimizing Eq.~\eqref{eq:inc_loss} using rays from multiple frames, we obtain more accurate reconstruction of the surface as shown in Figure~\ref{fig:5frames_w_reg}, where the reconstruction of the low-textured surface is driven by $\loss_\seg$ and $\loss_\reg$.

% Our regularization is similar to the term used in previous works \cite{nerf_w, neuraldiff} but with an additional multiplicative term that forces the reconstruction near the origin.

% \begin{figure*}[h!tb]
%     \begin{center}
%         \begin{minipage}{.19\linewidth}
%         \centering
%         {\includegraphics[width=1\linewidth]{figures/reg_term/no_reg_batchsize1/00740_real.png}}
%         % {\includegraphics[page=2,trim=140 105 170 40, clip, width=1\linewidth]{figures/reg_term/reg_term.pdf}}

%         \subcaptionbox{Single Frame Real Depth}
%         {\includegraphics[trim=110 105 130 115, clip,width=1\linewidth]{figures/reg_term/no_reg_batchsize1/00740_view_rend_real.png}}
%         \end{minipage}~\vrule~%
%         %
%         %
%         \begin{minipage}{.19\linewidth}
%         \centering
%         {\includegraphics[width=1\linewidth]{figures/reg_term/no_reg_batchsize1/00740_pred.png}}

%         \subcaptionbox{Single Frame w/o Reg.\label{fig:1frame_wo_reg}}
%         {\includegraphics[trim=20 45 20 45, clip,width=1\linewidth]{figures/reg_term/no_reg_batchsize1/00740_occ_vis_pred.png}}
%         \end{minipage}~%
%         %
%         %
%         \begin{minipage}{.19\linewidth}
%         \centering
%         {\includegraphics[width=1\linewidth]{figures/reg_term/no_reg_batchsize5/00740_pred.png}}

%         \subcaptionbox{Five Frames w/o Reg.\label{fig:5frames_wo_reg}}
%         {\includegraphics[trim=20 35 00 35,clip, width=1\linewidth]{figures/reg_term/no_reg_batchsize5/00780_occ_vis_pred.png}}
%         \end{minipage}~%
%         %
%         %
%         \begin{minipage}{.19\linewidth}
%         \centering
%         {\includegraphics[width=1\linewidth]{figures/reg_term/reg_batchsize1/00740_pred.png}}

%         \subcaptionbox{Single Frame w/ Reg.\label{fig:1frame_w_reg}}
%         {\includegraphics[trim=90 120 150 100, clip,width=1\linewidth]{figures/reg_term/reg_batchsize1/00740_occ_vis_pred.png}}
%         \end{minipage}~%
%         %
%         %
%         \begin{minipage}{.19\linewidth}
%         \centering
%         {\includegraphics[width=1\linewidth]{figures/reg_term/reg_batchsize5/00740_pred.png}}

%         \subcaptionbox{Five Frames w/ Reg.\label{fig:5frames_w_reg}}
%         {\includegraphics[trim=20 60 00 20, clip,width=1\linewidth]{figures/reg_term/reg_batchsize5/00780_occ_vis_pred.png}}
%         \end{minipage}~%
%         %
%         %
%     \end{center}
%     \vspace{-0.5cm}
%     \caption{In the top row, we show segmented RGB image of the object (a), and the rendered images of the object (b-e) with different settings. In the bottom row, we show the top view of the camera and the point cloud of the object using real depth (a), and the occupancy field obtained from our method under different settings (b-e). The occupancy field obtained without our regularization term with one or five frames is distorted (b,c), more so in the low-texture regions. When using the regularization term with a single frame (d), the occupancy field is mostly constrained to a plane parallel to the image plane (shown in green). With multiple frames and regularization term (e), we obtain more accurate reconstruction of the object surface. The cameras in red are the additional frames used in optimization.}
%     \label{fig:reg_term}
%     \vspace{-0.3cm}
% \end{figure*}

% \begin{figure}[t]
%     \centering
%     \includegraphics[trim=10 0 55 8, clip, width=1\linewidth]{figures/method/depth_err_no_depth.pdf}
%     \caption{Rendered color images and normalized depth error between rendered depth and ground-truth depth for a frame shown on the left at different tracking steps when the 3D loss term $\loss_\text{dep}$ is not used in tracking. The estimated and ground-truth trajectory of object pose is shown in the bottom row at different tracking steps. Without $\loss_\text{dep}$ the object shape undergoes large deformations during tracking affecting the estimated poses.}
%     \label{fig:no_depth}
% \end{figure}


% as shown in Figure~\ref{fig:5frames_w_reg}

% For tracking step $t=0$, we initialize all the camera poses corresponding to the frames in $\calS_0$ to the same pose positioning them at a certain distance from the origin and pointing towards the origin. As multiple frames are required to reconstruct the object surface, we add more than one frame in each step of the tracking process such that $\lvert\calS_i\rvert = N_\trac$, where $\lvert \cdot \rvert$ represents the cardinality of the set and $N_\trac>1$. \vincent{In practice, we use $N_\trac = ..$.}


% As every set of new frames during tracking refine the object surface, we optimize both the object shape and color, and poses of all the frames until the current tracking step as indicated in Eq.~\eqref{eq:inc_loss}. We also optimize the poses corresponding to frames in the previous tracking steps $\{\calS_i\}_{i=0}^{t-1}$ as they depend on the object shape. During optimization, we draw a fixed percentage of rays in a batch from the latest frames $\calS_t$ to ensure that the budget for rays required for reconstructing the incremental new surface remains constant.

% Our tracking procedure differs from the SLAM-type tracking such as IMAP~\cite{imap} which optimizes the pose of the latest frame while freezing the scene network ($\theta$ in our case) and the previously tracked poses in each tracking step. IMAP relies heavily on depth data which provides a strong supervision for accurately reconstructing the partial scene geometry even with just a single frame. In our case, due to absence of depth, the object geometry reconstructed at tracking step, $t=0$ may not always be reliable and hence need to be refined at every tracking step to avoid large drifts. 
% Thus, at each tracking step we optimize the object shape and color, and also optimize the poses of the previously tracked frames as they depend on the object shape. This results in effectively optimizing all the parameters $\theta$ and the poses of all the frames until the current tracking step as indicated in Eq.~(\ref{eq:inc_loss}). During optimization, we draw a fixed percentage of rays in a batch from the latest frames, $\calS_t$ to ensure that the budget for rays required for reconstructing the incremental new surface remains unchanged. Our tracking procedure is thus similar to `mapping' procedure in IMAP except for ray budget allocation and we avoid a separate mapping procedure.

% The ray budget allocation and \vincentrmk{what do you mean by: } non-uniform distribution of the poses of the object may result in uneven sampling of the rays around the object causing drift in poses and object shape during tracking as shown in Figure~\ref{fig:depth_term} (a-c). We thus introduce a depth loss term based on the rendered depths to constrain drift in object shape. We take it as

\shreyas{

\paragraph{Depth term $\loss_\dep^i$.}  We additionally use a loss term based on rendered depths to stabilize the tracking. This loss is only applied to rays from the frames that were previously tracked. After tracking each frame $i$, the depth map, $\hat{d}^i$ is rendered using the optimized pose and used in the future tracking steps using the term
%
\begin{equation}
    \loss_\dep^i = \big(d^i(\ray)-\hat{d}^i(\ray)\big)^2 \> ,
\end{equation}
%
where $d(\ray) = \sum_k \gamma(\bx_k) p_k$ is the estimated depth of the ray. $\gamma(\cdot)$ and $p_k$ are the blending coefficient and ray length defined in Section~\ref{sec:problem}.
\vincentrmk{Does 'depth of the ray' mean the same as 'length of the ray'?} \shreyasrmk{Yes, I think we need a better term to differentiate the two!}. Figure~\ref{fig:depth_term}(a-c) shows the reconstructed object and the estimated and ground-truth object trajectories without the depth loss term at three tracking steps. The object shape is distorted at step $t=5$ and the estimated poses are inaccurate as seen in step $t=9$. When using the depth term, the object shape and the tracked poses are more stable as shown in Figure~\ref{fig:depth_term}(d-f).}

\shreyasrmk{percentage of sampled rays in a batch}

% where $\bar{d}(\ray)$ is the pre-computed depth of the rayand $\hat{d}(\ray)$ is the depth of the ray obtained as $\hat{d}(\ray) = \sum_k \gamma(\bx_k) p_k$, where $\gamma(\cdot)$ and $p_k$ are as defined in Eq.~(\ref{eqn:rend_eqn}). Note that at each tracking step $t$, the depth loss term only applies to rays from all the frames in the previous tracking steps $\{\calS_i\}_{i=0}^{t-1}$ for which $\bar{d}$ can be pre-computed. After tracking step $t$, we only compute the depth for frames in $\calS_t$ to avoid re-rendering all the previous frames. We observe that such an approximation has little impact on the tracking accuracy. The depth loss term provides a way for `remembering' object shape reconstructed in the previous tracking steps. The complete tracking loss is defined as
%
% %
% \begin{equation}
%     \loss_\track = \loss_\inc + \loss_\dep \> .
% \end{equation}
% %
% Figure~\ref{fig:depth_term}(d-f) shows the result when using the depth term during tracking. The tracking is more stable with better reconstruction of the object when using $\loss_\text{dep}$.

\begin{figure}[t]
    % \begin{center}
        \begin{minipage}{.32\linewidth}
        \subcaptionbox{$t=0$, w/o $\loss_\text{dep}$}
        {\includegraphics[page=1,trim=170 50 140 35,clip,width=1\linewidth]{figures/method/depth_term2.pdf}}~\subcaptionbox{$t=5$, w/o $\loss_\text{dep}$}
        {\includegraphics[page=2,trim=170 50 140 35,clip,width=1\linewidth]{figures/method/depth_term2.pdf}}~\subcaptionbox{$t=9$, w/o $\loss_\text{dep}$}
        {\includegraphics[page=3,trim=170 50 140 35,clip,width=1\linewidth]{figures/method/depth_term2.pdf}}
        \end{minipage}
        
        \begin{minipage}{.32\linewidth}
        \centering
        \subcaptionbox{$t=0$, w/ $\loss_\text{dep}$}
        {\includegraphics[page=4,trim=170 50 140 35,clip,width=1\linewidth]{figures/method/depth_term2.pdf}}~\subcaptionbox{$t=5$, w/ $\loss_\text{dep}$}
        {\includegraphics[page=5,trim=170 50 140 35,clip,width=1\linewidth]{figures/method/depth_term2.pdf}}~\subcaptionbox{$t=9$, w/ $\loss_\text{dep}$}
        {\includegraphics[page=6,trim=170 50 140 35,clip,width=1\linewidth]{figures/method/depth_term2.pdf}}
        \end{minipage}
    % \end{center}
    % \vspace{-0.5cm}
    \caption{Effect of $\loss_\dep$ on object reconstruction visualized at three different tracking steps, $t=\{0,5,9\}$. The estimated and the ground-truth camera trajectories are shown in red and blue, respectively. The rendered image on the first camera of the estimated trajectory, shown in yellow, is displayed on the inset. $\loss_\dep$ provides more constraints on the occupancy field, which results in more stable tracking.}
    \label{fig:depth_term}
    \vspace{-0.3cm}
\end{figure}

% The losses introduced in Eq.~(\ref{eq:inc_loss}) are defined in 2D (except the regularization term) and does not provide enough constraints on the shape of the object during tracking. In Figure~\ref{fig:no_depth}, we visualize the reconstructed surface by comparing the rendered depth with the camera-captured depth after scale-normalization at different tracking steps for a given frame. Though the rendered images for the same frame at all tracking steps are similar to the input image (Figure~\ref{fig:no_depth}(a)) implying $\loss_\text{col}$ and $\loss_\text{seg}$ are minimized, the object shape is unconstrained and undergoes large variations (Figure~\ref{fig:no_depth}(b)) affecting the pose tracking (Figure~\ref{fig:no_depth}(c)).

% We constrain the object shape using the rendered depth maps, $\calD_i$ that are computed for the set of frames $\calS_i$ after each tracking step. The rendered-depth loss for the rays from previously tracked frames is defined as,
% \begin{equation}
%     \loss_\text{dep} = \sum_{\ray\in \{\calS_i\}_{i=0}^{t-1}} \big(\hat{d}(\ray)-\bar{d}(\ray)\big)^2,
% \end{equation}
% where, $\bar{d}(\ray)$ is the pre-computed depth of the ray and $\hat{d}(\ray)$ is the depth of the ray obtained using the rendering equation similar to Eq.~(\ref{eqn:rend_eqn}). Though $\bar{d}$ is not the accurate depth of the ray, it constrains the object shape from undergoing large deformations and provides a way for `remembering' the object shape reconstructed in the previous tracking steps. Our tracking loss thus constitutes both 2D and 3D terms and is defined as,
% \begin{equation}
%     \loss_\text{track} = \loss_\text{inc} + \loss_\text{dep}
% \end{equation}
% Figure~\ref{fig:with_depth} shows the normalized depth error and pose trajectories using the above tracking loss, $\loss_\text{track}$. The tracking is more stable with depth loss, $\loss_\text{dep}$.

% \begin{figure}[t]
%     \centering
%     \includegraphics[trim=50 0 55 8, clip, width=1\linewidth]{figures/method/depth_err_with_depth.pdf}
%     \caption{Rendered color images and normalized depth error between rendered depth and ground-truth depth for the frame shown in Figure~\ref{fig:no_depth} at different tracking steps when the 3D loss term $\loss_\text{dep}$ is used in tracking. The estimated and ground-truth trajectory of object pose is shown in the bottom row at different tracking steps. $\loss_\text{dep}$ results in more stable tracking while constraining the shape of the object.}
%     \label{fig:with_depth}
% \end{figure}

% \subsection{Inter-segment optimization}
\subsection{Global optimization}
\label{sec:stitch}

% \vincentrmk{in general, avoid the passive form and "jargon". 
% "the  poses in each segment are scale-normalized" $\rightarrow$ 
% "We normalize the poses so that the camera trajectories get the same scale"}


We define the neighboring video segments so that they overlap over a few frames: The camera trajectories and object reconstruction for each segment are recovered up to a rigid motion and scale factor, and these shared frames allow us to express them into a unique coordinate frame. We thus normalise the camera poses to give the camera trajectories the same scale before combining two segments. 

We achieve this with the following procedure. 
Let $\campose_i^k =[\phi_i; t_i]$ be the rotation and translation of the camera for the $i^\text{th}$ frame in segment $k$ with $N_s$ frames. We obtain a normalized pose by taking $\hat{\campose}_i^k = \big[\phi_i; t_i/\frac{1}{N_s}\sum_j \|t_j\|\big]$. 
\vincentrmk{I am surprised that works. This assumes that the object remains at the same distance from the camera for the 2 segments, no?}
We then retrieve the rigid motion $\campose$~(rotation and translation) that aligns the camera poses for the frames shared 
by the two segments:
% The camera poses of the overlapping frames in the segment $k$ are SE(3) transformed to align with frames in the neighboring segment, $\calN(k)$ using the matrix, $\campose_{k\rightarrow\calN(k)}$ obtained as
%
\begin{equation}
    \campose_{k\rightarrow\calN(k)} = \arg\min_\campose \sum_i \|\campose\cdot\hat{\campose}_i^k-\hat{\campose}_i^{\calN(k)}\|_F \> ,
\end{equation}
%
where $\|\cdot\|_F$ denotes the Frobenius norm and the summation is over the set of overlapping frames. In practice, we observed that as less as a single overlapping frame is sufficient for combining the segments.

\vincent{
Finally, we optimize the loss function in Eq.~\eqref{eq:first_loss} over all the frames of all the segments, starting from the cameras to combine the segments
The cameras are initialized with the unit-scale normalized poses and the loss function defined in Eq.~\eqref{eq:first_loss} is optimized to combine the segments. The network parameters $\theta$ are initialized to reconstruct a sphere. Pairs of neighboring segments are iteratively combined until the object is reconstructed from the full sequence.
}

==> old_method.tex <==
\section{Problem Formulation}
\label{sec:problem}

% in this section, we formalize/..

\vincentrmk{It is weird to introduce campose using its inverse ($\campose_i^{-1}$). Isnt it more logical to talk about object pose rather than cam pose here?}\shreyasrmk{If we introduce the object pose, we will need to invert it everytime in the equations later. I tried introducing campose directly below}

\vincentrmk{We should postpone the introduction of notations and equations as much as possible anyway}\shreyasrmk{Will work on this}

\vincent{
Our setup for simultaneous object reconstruction and tracking consists of a static RGB camera and an unknown rigid object being scanned by one or two hands in the field of view of the camera under static lighting conditions. \shreyas{We denote the $N$ images in the captured sequence by $\{\calI_i\}_{i=1}^N$, and the pose of the camera in the object coordinate system at frame $i$ by $\campose_i$. We assume a static background whose image is either obtained separately or is estimated from the sequence using the segmentation masks of hand and object.}
% We discard the background and hand in each image by segmenting them using  by off-the-shelf networks\vincentrmk{we need more details here} and setting them to black. 
}
\vincentrmk{I understand what you mean but this can be a bit confusing. Do we need it? :}\shreyasrmk{The other way is to describe everything in the camera coordinate system (right now all the equations are in object coordinate system). I think people are used to seeing nerf rendering equations in the object coordinates and changing this to camera coordinates may make them look complex? Fig.2 is great, how about I refine it a little bit and refer to it for this interpretation?} \vincentrmk{Sure, do not hesitate to change it}
The resulting images can be seen as images of the rigid object captured from multiple views with a fixed relative transformation between the camera and the light sources. 

Similarly to UNISURF~\cite{unisurf}, we represent the object to reconstruct by an occupancy field network and a color field network at every 3D point and aim to find the optimal parameters for these two networks. 
There is however a very important difference: Standard NeRF methods~\cite{nerf, unisurf, other_nerf_papers} work under the assumption of a static scene and light environment and varying camera locations. This allows these methods to condition the color field only on the viewing ray in the scene coordinate system to capture non-Lambertian surfaces. 


In our case, as the camera and the light sources with their relative poses fixed capture the static object from different views, we also need to condition the color field on the ray \emph{length}.
\vincentrmk{Isnt this because the rays are defined in the camera coordinate system?  What happens if you consider rays in the object coordinate system?  We should probably discuss the alternatives.}

%Similar to \cite{unisurf}, we represent the object to be reconstructed by an occupancy field network $o_\theta(\bx)$ and the color field network $c_\theta(\bx)$ at every 3D point, $\bx$, and aim to find the optimal network parameters $\theta$. Traditional NeRF methods~\cite{nerf, unisurf, other_nerf_papers} that work under the assumption of static scene and light setup, but varying camera locations condition the color field on the viewing direction, $\bd$ to model non-Lambertian surfaces. In our case, as the camera and the light sources with their relative poses fixed capture the static object from different views, we model the color field also conditioned on the ray length. 

This is illustrated in Figure~\ref{fig:raydist}: When a 3D point on the object surface is viewed by the camera under two different object poses, its color may change even if the direction of the line of sight remains the same. This is because the angle between the line of sight and the light direction changes, and the amount of light reflected toward the camera is a function of this angle. A simple way to capture this phenomenon is to condition the color field on the distance between the camera and the 3D point.

\vincentrmk{this does not capture everything, no?  The color also depends on the normal. If the object rotates around the point, the ray direction and length and light direction do not change but the normal changes, which will change the point's color.  Maybe it does not matter because it does not happen in practice? }

shows an example of a point on the object surface viewed by a camera at two different poses of the object relative to the camera such that the viewing direction is the same. A point-light source located at a fixed position, $\calM$ w.r.t to the camera results in two different incident light directions and is a function of viewing direction, ray length and camera position $\calM$. Our color field $c_\theta(\bx,\bd,p)$ is thus conditioned on view direction, $\bd$ and ray length, $p$ as $\calM$ is constant in all the images. \vincentrmk{Maybe $c$ should be bold since it is a (color) vector?}

% \begin{figure}
%     \centering
%     \includegraphics[trim=100 180 400 100, clip, ,width=1\linewidth]{figures/method/ray_dist.pdf}
%     \caption{Incident and reflected rays under two different poses of the object relative to the camera. The relative position between the camera and the point-light does not change during the capture. The observed object color is  dependent both on the viewing ray direction and the ray length as the object changes its pose while the camera and the light source remain static.}
%     \label{fig:raydist}
% \end{figure}


\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{figures/ray_length.png}
    \caption{Top: In the case of the standard NeRF setting, the camera moves with respect to the scene, and the color of a 3D point depends only on the direction of the light of sight. Bottom: In the case of in-hand scanning, the object moves with respect to the camera and the lights, and the color of a 3D point on the surface of the object does not depend only on the direction of the light of sight but also on the object pose. To capture this, we simply condition the color of the point on the distance between the camera and the point, in addition to the direction of the line of sight. \vincentrmk{figure is pretty ugly, but gives a better idea I think}}
    \label{fig:raydist}
\end{figure}

\vincent{
A second major difference with other NeRF approaches is that we need to estimate the camera pose with respect to the object, while previous approaches often assume the camera poses to be given. We thus estimate the object's shape and appearance by solving:
%
\begin{align}
    \label{eq:complete_loss}
    \theta^*, \{\campose_i^*\}_{i=1}^N &= \arg\min_{\theta, \{\campose_i\}_{i=1}^N} \sum_j \sum_{\ray\in \calR_j} \Big(\loss_\text{col}(\ray)+\loss_\text{seg}(\ray)\Big) \> .
\end{align}
%
$\theta$ denotes the parameters of the neural surface, and the $\campose_i$s are the camera poses in the object coordinate system\vincentrmk{Is that correct?} for the sequence. $\calR_j$ is the set of rays for frame $j$.

Term $\loss_\text{col}(\ray)$ is a loss on the predicted color for ray $\ray$: 
%
\begin{align}
    \label{eq:col_loss}
    \loss_\text{col}(\ray) &= \|\hat{C}(\ray) - C(\ray)\|_2 \> .
\end{align}
%
where $\hat{C}(\ray)$ is the predicted color for ray $\ray$ and $C(\ray)$ is its observed color. For $\hat{C}(\ray)$, we follow the rendering equation of UNISURF:
%
\begin{align}
\label{eqn:rend_eqn}
    \hat{C}(\ray) &= \sum_{k=1}^M \gamma(\bx_k) c_\theta(\bx_k,\bd,p_k) \> .
\end{align}
%
$c_\theta(\bx_k,\bd,p_k)$ is the neural color field for point $\bx_k$ sampled along ray $\ray$, seen under the direction $\bd$ of ray $\ray$, and with distance $p_k$ from the camera center for frame $j$. \vincentrmk{Do we really need $\campose$ in $c$?}  $\gamma(\bx_k)$ is the \vincentrmk{Does gamma have a name? visibility maybe?} and is computed as
%
\begin{align}
\label{eqn:gamma}
    \gamma(\bx_k) &= o_\theta(\bx_k) \prod_{l<k} \big(1-o_\theta(\bx_l)\big) \> ,
\end{align}
%
\vincentrmk{do gamma and $o$ really depend on the camera pose?}
where $o_\theta(\bx_{k,i};\campose_i)$ is the \vincentrmk{? neural occupancy field?}.

The second term $\loss_\text{seg}(\ray)$ in Eq.~\eqref{eq:complete_loss} is a ``segmentation loss'' for ray $\ray$:
%
\begin{align}
    \label{eq:seg_loss}
    \loss_\text{seg}(\ray) &= \text{BCE}\Big(\max_k~\{o_\theta(\bx_k)\}, S_o(\ray) \Big) \> ,
\end{align}
%
\vincentrmk{there is no campose in $o$ in this equation}
where $\text{BCE}(\cdot)$ is the binary cross-entropy loss, and $S_o(\ray)$ is the observed object segmentation value for ray $\ray$: Remember that we segment hand and background to keep only the object in the images. $S_o(\ray)$ is equal to 1 if the ray projects on the object as estimated by the segmentation, and 0 otherwise.  $\max_k~\{o_\theta(\bx_k)\}$ is the maximum occupancy along ray $\ray$, which should also be equal to 1 if the ray intersects the object and to 0 otherwise.

We detail in the next section how we solve Eq.~\eqref{eq:complete_loss}.


% and $\loss_\text{seg}(\ray)$ is a segmentation loss for the ray $\ray$ respectively, $C(\ray)$ is the observed color of ray $\ray$, $\calR$ is the set of all pixels in all the frames, $BCE(\cdot)$ is the binary cross-entropy loss, and $S_o(\ray)$ is the observed object segmentation value for the ray $\ray$. We drop the dependency of $\hat{C}$ on the pose, $\campose$ for brevity.

% We drop the dependency of $\hat{C}$ on the pose, $\campose$ for brevity.

}

% We follow the rendering equation described in UNISURF~\cite{unisurf} to perform volumetric rendering with $M$ 3D points $\{\bx_{k,i}\}_i$ sampled along the ray, $\ray_k=\bo(\campose_k)+t\bd(\campose_k)$ originating from the camera $k$ whose pose is $\campose_k$, camera center is $\bo(\campose_k)$ and the ray direction is $\bd(\campose_k)$. The coordinates $\bx_i^k$, ray direction $\bd$ and ray length, $p_i = \|\bx_i^k-\bo(\campose_k)\|_2$ are encoded using the sinusoidal representation~\cite{unisurf} and the rendering equation is given by
% %
% \begin{align}
% \label{eqn:rend_eqn}
%     \hat{C}(\ray_k;\campose_k) &= \sum_{i=1}^M \gamma(\bx_{k,i};\campose_k) ~c_\theta(\bx_{k,i},\bd,p_i;\campose_k),\\
%     \gamma(\bx_{k,i};\campose_k) &= o_\theta(\bx_{k,i};\campose_k) \prod_{j<i} \big(1-o_\theta(\bx_{k,i};\campose_k)\big)
% \end{align}
% %
% where $\hat{C}$ is the rendered pixel value. The parameters $\theta^*$ representing the object and the camera poses $\{\campose_i^*\}_{i=1}^N$ is given by
% %
% \begin{align}
%     \label{eq:first_loss}
%     \theta^*, \{\campose_i^*\}_{i=1}^N &= \arg\min_{\theta, \{\campose_i\}_{i=1}^N} \sum_{\ray\in \calR} \Big(\loss_\text{col}(\ray)+\loss_\text{seg}(\ray)\Big) \\
%     \loss_\text{col}(\ray) &= \|\hat{C}(\ray) - C(\ray)\|_2\nonumber \\
%     \loss_\text{seg}(\ray) &= BCE\Big(\max_i~\{o_\theta(\bx_{k,i})\}, S_o(\ray) \Big) \nonumber,
% \end{align}
% %
% where $\loss_\text{col}(\ray)$ and $\loss_\text{seg}(\ray)$ are the RGB color loss and segmentation loss for the ray $\ray$ respectively, $C(\ray)$ is the observed color of ray $\ray$, $\calR$ is the set of all pixels in all the frames, $BCE(\cdot)$ is the binary cross-entropy loss, and $S_o(\ray)$ is the observed object segmentation value for the ray $\ray$. We drop the dependency of $\hat{C}$ on the pose, $\campose$ for brevity.




%We follow the rendering equation described in UNISURF~\cite{unisurf} to perform volumetric rendering with $M$ 3D points $\{\bx_{k,i}\}_i$ sampled along the ray, $\ray_k=\bo(\campose_k)+t\bd(\campose_k)$ originating from the camera $k$ whose pose is $\campose_k$, camera center is $\bo(\campose_k)$ and the ray direction is $\bd(\campose_k)$. The coordinates $\bx_i^k$, ray direction $\bd$ and ray length, $p_i = \|\bx_i^k-\bo(\campose_k)\|_2$ are encoded using the sinusoidal representation~\cite{unisurf} and the rendering equation is given by
% %
% \begin{align}
% \label{eqn:rend_eqn}
%     \hat{C}(\ray_k;\campose_k) &= \sum_{i=1}^M \gamma(\bx_{k,i};\campose_k) ~c_\theta(\bx_{k,i},\bd,p_i;\campose_k),\\
%     \gamma(\bx_{k,i};\campose_k) &= o_\theta(\bx_{k,i};\campose_k) \prod_{j<i} \big(1-o_\theta(\bx_{k,i};\campose_k)\big)
% \end{align}
% %
% where $\hat{C}$ is the rendered pixel value. The parameters $\theta^*$ representing the object and the camera poses $\{\campose_i^*\}_{i=1}^N$ is given by
% %
% \begin{align}
%     \label{eq:first_loss}
%     \theta^*, \{\campose_i^*\}_{i=1}^N &= \arg\min_{\theta, \{\campose_i\}_{i=1}^N} \sum_{\ray\in \calR} \Big(\loss_\text{col}(\ray)+\loss_\text{seg}(\ray)\Big) \\
%     \loss_\text{col}(\ray) &= \|\hat{C}(\ray) - C(\ray)\|_2\nonumber \\
%     \loss_\text{seg}(\ray) &= BCE\Big(\max_i~\{o_\theta(\bx_{k,i})\}, S_o(\ray) \Big) \nonumber,
% \end{align}
% %
% where $\loss_\text{col}(\ray)$ and $\loss_\text{seg}(\ray)$ are the RGB color loss and segmentation loss for the ray $\ray$ respectively, $C(\ray)$ is the observed color of ray $\ray$, $\calR$ is the set of all pixels in all the frames, $BCE(\cdot)$ is the binary cross-entropy loss, and $S_o(\ray)$ is the observed object segmentation value for the ray $\ray$. We drop the dependency of $\hat{C}$ on the pose, $\campose$ for brevity.


\section{Method}


% 1 paragraph to explain the challenges of solving the pb

% 1 paragraph with an overview of how you solve these challenges

As the object undergoes a large motion in 3D during scanning, solving Eq.~\eqref{eq:full_loss} requires coarse initialization of the camera poses: As we show later in our experiments, random or fixed initialization of the pose parameters followed by optimization similar to BARF~\cite{barf} leads to degenerate solutions. Though COLMAP~\cite{colmap} is the standard method for obtaining coarse level pose estimates in NeRF-based methods~\cite{nerf,nerf_w,nerv,nerd}, it fails to obtain sufficient keypoint matches that are necessary for pose estimation in the regions of the object that contain less texture. As a result, COLMAP can provide reliable pose initialization only for highly-textured objects. 

Our approach to reconstruction of generic objects (both textured and non-textured) and their pose estimation is based on tracking, which incrementally reconstructs the object surface while simultaneously optimizing the poses at each tracking step. As tracking algorithms suffer from drift~\cite{}, we divide the video sequence into multiple overlapping segments and reconstruct parts of the object surface and obtain pose estimates within each segment independently. Finally, using the camera poses obtained in each segment, the segments are \textit{stitched} together and a global optimization similar to Eq.~\eqref{eq:first_loss} is performed to achieve complete object reconstruction. We provide details about the intra-segment tracking, inter-segment optimization and the algorithm for dividing the video sequence into multiple segments below.

\subsection{Intra-Sequence Segment Tracking}
\label{sec:tracking_method}

Let $\calS_t$ denote the set of new frames from the sequence that are added at tracking step $t$. $\{\calS_i\}_{i=0}^{t-1}$ denotes the set of frames which are used for tracking in the previous $t-1$ steps. The poses of the cameras corresponding to frames in $\calS_t$ are initialized using the second-order motion model on the trajectory of the poses of $\{\calS_i\}_{i=0}^{t-1}$. The occupancy and color network parameters, $\theta$, at step $t$ are initialized from the previous tracking step $t-1$. Further, after each tracking step $t$, we render and store the set of depth maps, $\calD_t$ in the views $\calS_t$ using the optimized poses. 

The optimization at each tracking step is intended to update the network parameters, $\theta$, such that,
\begin{itemize}
    \item the updated parameters also represent the incremental new surface visible in views $\calS_t$.
    \item the object surface reconstructed in the previous views $\{\calS_i\}_{i=0}^{t-1}$ is intact and not \textit{forgotten}
\end{itemize}
The incremental surface visible in $\calS_t$ is reconstructed by minimizing the objective function,
%
%
\begin{equation}
\label{eq:inc_loss}
    \loss_\text{inc} = \sum_{\ray\in\{\calS_i\}_{i=0}^t} \loss_\text{col}(\ray) + \loss_\text{seg}(\ray) + \loss_\text{opf}(\ray) + \loss_\text{reg}(\ray) \> ,
\end{equation}
%
where the former two terms $\loss_\text{col}$ and $\loss_\text{seg}$ are color and segmentation losses as defined in Eq.~\eqref{eq:first_loss}, and the latter two terms $\loss_\text{ofp}$ and $\loss_\text{reg}$ are the optical flow loss and the regularization term. We provide more details about the latter two terms below.

\paragraph{Optical Flow Loss, $\loss_\text{opf}$}This term provides additional constraint for the camera poses and is defined as,
%
\begin{align}
    \loss_\text{opf}(\ray_k) = \sum_i &\Big(\pi\big( \campose_{\calN(k)}  \bx_{k,i}\big) - \pi\big( \campose_k  \bx_{k,i}\big) - OF_{\ray_k}\Big) \cdot \nonumber \\ 
    &\gamma(\bx_{k,i};\campose_k), \nonumber
\end{align}
%
where $\ray_k$ is the ray from the $k^\text{th}$ frame, $\{\bx_{k,i}\}_i$ are the samples along the ray $\ray_k$, $\campose_{\calN(k)}$ is the pose of the frame that is neighboring the frame $k$ with pose $\campose_k$, $\pi(\cdot)$ is the camera projection function, and $OF_{\ray_k}$ is the optical flow precomputed at pixel/ray $\ray_k$.

\paragraph{Regularization Term, $\loss_\text{reg}$}Minimizing Eq.~(\ref{eq:inc_loss}) using rays from one or more frames without the regularization term results in degenerate solutions as shown by the occupancy fields in Figure~\ref{fig:1frame_wo_reg} and Figure~\ref{fig:5frames_wo_reg}. The distortion mainly occurs in low-texture regions, such as bottom of the $\textit{power\_drill}$ object in Figure~\ref{fig:reg_term} where $\loss_\text{col}$ cannot provide meaningful gradients to optimize the poses, while the rendered images are still reasonable. 

We introduce regularizer on the occupancy field to avoid degenerate solutions and is defined as,
\begin{equation}
\label{eq:reg_loss}
    \loss_\text{reg}(\ray_k) = \sum_i o_\theta(\bx_{k,i}) \exp{(\alpha \cdot \|\bx_{k,i}\|_2)},
\end{equation}
%
where, $\alpha$ is a hyper-parameter. $\loss_\text{reg}$ ensures that the object is reconstructed near the origin of the coordinate system and discourages artifacts in the occupancy field. When considering rays from a single camera located at a certain distance from the origin and pointing towards the origin, $\loss_\text{reg}$ forces reconstruction of the object surface on a plane that is nearly parallel to the image plane and passing through the origin as shown in Figure~\ref{fig:1frame_w_reg}. This can be proved by considering an orthographic projection of the rays and noting that for each ray, $\ray_k$, $o_\theta(\bx_{k,i}) = \{0,1\}$~\cite{unisurf} and $\loss_\text{reg}(\ray_k)$ is minimized when $\|\bx_{k,i}\|$ is minimized, which is a point on a plane perpendicular to the ray direction and passing through the origin. When minimizing Eq.~(\ref{eq:inc_loss}) using rays from multiple frames, we obtain more accurate reconstruction of the surface as shown in Figure~\ref{fig:5frames_w_reg}, where the reconstruction of the low-textured surface is driven by $\loss_\text{seg}$ and $\loss_\text{reg}$.

% Our regularization is similar to the term used in previous works \cite{nerf_w, neuraldiff} but with an additional multiplicative term that forces the reconstruction near the origin.

% \begin{figure*}[h!tb]
%     \begin{center}
%         \begin{minipage}{.19\linewidth}
%         \centering
%         {\includegraphics[width=1\linewidth]{figures/reg_term/no_reg_batchsize1/00740_real.png}}
%         % {\includegraphics[page=2,trim=140 105 170 40, clip, width=1\linewidth]{figures/reg_term/reg_term.pdf}}

%         \subcaptionbox{Single Frame Real Depth}
%         {\includegraphics[trim=110 105 130 115, clip,width=1\linewidth]{figures/reg_term/no_reg_batchsize1/00740_view_rend_real.png}}
%         \end{minipage}~\vrule~%
%         %
%         %
%         \begin{minipage}{.19\linewidth}
%         \centering
%         {\includegraphics[width=1\linewidth]{figures/reg_term/no_reg_batchsize1/00740_pred.png}}

%         \subcaptionbox{Single Frame w/o Reg.\label{fig:1frame_wo_reg}}
%         {\includegraphics[trim=20 45 20 45, clip,width=1\linewidth]{figures/reg_term/no_reg_batchsize1/00740_occ_vis_pred.png}}
%         \end{minipage}~%
%         %
%         %
%         \begin{minipage}{.19\linewidth}
%         \centering
%         {\includegraphics[width=1\linewidth]{figures/reg_term/no_reg_batchsize5/00740_pred.png}}

%         \subcaptionbox{Five Frames w/o Reg.\label{fig:5frames_wo_reg}}
%         {\includegraphics[trim=20 35 00 35,clip, width=1\linewidth]{figures/reg_term/no_reg_batchsize5/00780_occ_vis_pred.png}}
%         \end{minipage}~%
%         %
%         %
%         \begin{minipage}{.19\linewidth}
%         \centering
%         {\includegraphics[width=1\linewidth]{figures/reg_term/reg_batchsize1/00740_pred.png}}

%         \subcaptionbox{Single Frame w/ Reg.\label{fig:1frame_w_reg}}
%         {\includegraphics[trim=90 120 150 100, clip,width=1\linewidth]{figures/reg_term/reg_batchsize1/00740_occ_vis_pred.png}}
%         \end{minipage}~%
%         %
%         %
%         \begin{minipage}{.19\linewidth}
%         \centering
%         {\includegraphics[width=1\linewidth]{figures/reg_term/reg_batchsize5/00740_pred.png}}

%         \subcaptionbox{Five Frames w/ Reg.\label{fig:5frames_w_reg}}
%         {\includegraphics[trim=20 60 00 20, clip,width=1\linewidth]{figures/reg_term/reg_batchsize5/00780_occ_vis_pred.png}}
%         \end{minipage}~%
%         %
%         %
%     \end{center}
%     \vspace{-0.5cm}
%     \caption{In the top row, we show segmented RGB image of the object (a), and the rendered images of the object (b-e) with different settings. In the bottom row, we show the top view of the camera and the point cloud of the object using real depth (a), and the occupancy field obtained from our method under different settings (b-e). The occupancy field obtained without our regularization term with one or five frames is distorted (b,c), more so in the low-texture regions. When using the regularization term with a single frame (d), the occupancy field is mostly constrained to a plane parallel to the image plane (shown in green). With multiple frames and regularization term (e), we obtain more accurate reconstruction of the object surface. The cameras in red are the additional frames used in optimization.}
%     \label{fig:reg_term}
%     \vspace{-0.3cm}
% \end{figure*}

\begin{figure*}[h!tb]
    \begin{minipage}{.19\linewidth}
    \centering
    \subcaptionbox{Single Frame Real Depth}
    {\includegraphics[page=1,trim=140 105 170 40, clip, width=1\linewidth]{figures/reg_term/reg_term2.pdf}}~\vrule~%
    \subcaptionbox{Single Frame w/o Reg.\label{fig:1frame_wo_reg}}
    {\includegraphics[page=2,trim=140 105 170 40, clip, width=1\linewidth]{figures/reg_term/reg_term2.pdf}}~%
    \subcaptionbox{Five Frames w/o Reg.\label{fig:5frames_wo_reg}}
    {\includegraphics[page=3,trim=140 105 170 40, clip, width=1\linewidth]{figures/reg_term/reg_term2.pdf}}~%
    \subcaptionbox{Single Frame w/ Reg.\label{fig:1frame_w_reg}}
    {\includegraphics[page=4,trim=140 105 170 40, clip, width=1\linewidth]{figures/reg_term/reg_term2.pdf}}~%
    \subcaptionbox{Five Frames w/ Reg.\label{fig:1frame_w_reg}}
    {\includegraphics[page=5,trim=140 105 170 40, clip, width=1\linewidth]{figures/reg_term/reg_term2.pdf}}
    \end{minipage}
    % \vspace{-0.5cm}
    \caption{Visualization of the top view of the camera and the point cloud of the object using real depth (a), and the occupancy field obtained from our method under different settings (b-e). The occupancy field obtained without our regularization term with one or five frames is distorted (b,c), more so in the low-texture regions of the object (bottom part of $\textit{power\_drill}$). When using the regularization term with a single frame (d), the occupancy field is mostly constrained to a plane parallel to the image plane (shown in green). With multiple frames and regularization term (e), we obtain more accurate reconstruction of the object surface. The images rendered on to the cameras in black in each setting is shown on the inset.}
    \label{fig:reg_term}
    \vspace{-0.3cm}
\end{figure*}

% \begin{figure}[t]
%     \centering
%     \includegraphics[trim=10 0 55 8, clip, width=1\linewidth]{figures/method/depth_err_no_depth.pdf}
%     \caption{Rendered color images and normalized depth error between rendered depth and ground-truth depth for a frame shown on the left at different tracking steps when the 3D loss term $\loss_\text{dep}$ is not used in tracking. The estimated and ground-truth trajectory of object pose is shown in the bottom row at different tracking steps. Without $\loss_\text{dep}$ the object shape undergoes large deformations during tracking affecting the estimated poses.}
%     \label{fig:no_depth}
% \end{figure}

For the tracking step, $t=0$, the camera poses corresponding to the frames $\calS_0$ are all initialized to the same pose positioning them at a certain distance from the origin and pointing towards the origin. As multiple frames are required to reconstruct the object surface as shown in Figure~\ref{fig:5frames_w_reg}, we add more than one frame in each step of the tracking process such that $\lvert\calS_i\rvert = N_\text{trac}$, where $\lvert \cdot \rvert$ represents cardinality of the set and $N_\text{trac}>1$.

As every set of new frames during tracking refine the object surface, we optimize both the object shape and color, and poses of all the frames until the current tracking step as indicated in Eq.~(\ref{eq:inc_loss}). The poses corresponding to frames in the previous tracking steps $\{\calS_i\}_{i=0}^{t-1}$ are also optimized as they depend on the object shape. During optimization, we draw a fixed percentage of rays in a batch from the latest frames, $\calS_t$ to ensure that the budget for rays required for reconstructing the incremental new surface remains unchanged.

% Our tracking procedure differs from the SLAM-type tracking such as IMAP~\cite{imap} which optimizes the pose of the latest frame while freezing the scene network ($\theta$ in our case) and the previously tracked poses in each tracking step. IMAP relies heavily on depth data which provides a strong supervision for accurately reconstructing the partial scene geometry even with just a single frame. In our case, due to absence of depth, the object geometry reconstructed at tracking step, $t=0$ may not always be reliable and hence need to be refined at every tracking step to avoid large drifts. 
% Thus, at each tracking step we optimize the object shape and color, and also optimize the poses of the previously tracked frames as they depend on the object shape. This results in effectively optimizing all the parameters $\theta$ and the poses of all the frames until the current tracking step as indicated in Eq.~(\ref{eq:inc_loss}). During optimization, we draw a fixed percentage of rays in a batch from the latest frames, $\calS_t$ to ensure that the budget for rays required for reconstructing the incremental new surface remains unchanged. Our tracking procedure is thus similar to `mapping' procedure in IMAP except for ray budget allocation and we avoid a separate mapping procedure.

The ray budget allocation and non-uniform distribution of the poses of the object may result in uneven sampling of the rays around the object causing drift in poses and object shape during tracking as shown in Figure~\ref{fig:depth_term} (a-c). We introduce a depth loss term based on the rendered depths to constrain drift in object shape and is defined as
%
\begin{equation}
    \loss_\text{dep} = \sum_{\ray\in \{\calS_i\}_{i=0}^{t-1}} \big(\hat{d}(\ray)-\bar{d}(\ray)\big)^2,
\end{equation}
%
where, $\bar{d}(\ray)$ is the pre-computed depth of the ray and $\hat{d}(\ray)$ is the depth of the ray obtained as $\hat{d}(\ray) = \sum_i \gamma(\bx_i) p_i$, where $\gamma(\cdot)$ and $p_i$ are as defined in equation Eq.~(\ref{eqn:rend_eqn}). Note that at each tracking step $t$, the depth loss term only applies to rays from all the frames in the previous tracking steps $\{\calS_i\}_{i=0}^{t-1}$ for which $\bar{d}$ can be pre-computed. After tracking step $t$, we only compute the depth for frames in $\calS_t$ to avoid re-rendering all the previous frames. We observe that such an approximation has little impact on the tracking accuracy. The depth loss term provides a way for `remembering' object shape reconstructed in the previous tracking steps and overall tracking loss is defined as
%
%
\begin{equation}
    \loss_\text{track} = \loss_\text{inc} + \loss_\text{dep} \> .
\end{equation}
%
Figure~\ref{fig:depth_term} (d-f) shows the result when using the depth term during tracking. The tracking is more stable with better reconstruction of the object when using $\loss_\text{dep}$.

\begin{figure}[t]
    % \begin{center}
        \begin{minipage}{.32\linewidth}
        \subcaptionbox{$t=0$, w/o $\loss_\text{dep}$}
        {\includegraphics[page=1,trim=170 50 140 35,clip,width=1\linewidth]{figures/method/depth_term2.pdf}}~\subcaptionbox{$t=5$, w/o $\loss_\text{dep}$}
        {\includegraphics[page=2,trim=170 50 140 35,clip,width=1\linewidth]{figures/method/depth_term2.pdf}}~\subcaptionbox{$t=9$, w/o $\loss_\text{dep}$}
        {\includegraphics[page=3,trim=170 50 140 35,clip,width=1\linewidth]{figures/method/depth_term2.pdf}}
        \end{minipage}
        
        \begin{minipage}{.32\linewidth}
        \centering
        \subcaptionbox{$t=0$, w/ $\loss_\text{dep}$}
        {\includegraphics[page=4,trim=170 50 140 35,clip,width=1\linewidth]{figures/method/depth_term2.pdf}}~\subcaptionbox{$t=5$, w/ $\loss_\text{dep}$}
        {\includegraphics[page=5,trim=170 50 140 35,clip,width=1\linewidth]{figures/method/depth_term2.pdf}}~\subcaptionbox{$t=9$, w/ $\loss_\text{dep}$}
        {\includegraphics[page=6,trim=170 50 140 35,clip,width=1\linewidth]{figures/method/depth_term2.pdf}}
        \end{minipage}
    % \end{center}
    % \vspace{-0.5cm}
    \caption{Effect of $\loss_\text{dep}$ on object reconstruction visualized at three different tracking steps, $t=\{0,5,9\}$. The estimated and the ground-truth camera trajectory are shown in red and blue, respectively. The rendered image on the first camera of the estimated trajectory, shown in yellow is displayed on the inset. $\loss_\text{dep}$ provides more constraints on the occupancy field resulting in more stable tracking.}
    \label{fig:depth_term}
    \vspace{-0.3cm}
\end{figure}

% The losses introduced in Eq.~(\ref{eq:inc_loss}) are defined in 2D (except the regularization term) and does not provide enough constraints on the shape of the object during tracking. In Figure~\ref{fig:no_depth}, we visualize the reconstructed surface by comparing the rendered depth with the camera-captured depth after scale-normalization at different tracking steps for a given frame. Though the rendered images for the same frame at all tracking steps are similar to the input image (Figure~\ref{fig:no_depth}(a)) implying $\loss_\text{col}$ and $\loss_\text{seg}$ are minimized, the object shape is unconstrained and undergoes large variations (Figure~\ref{fig:no_depth}(b)) affecting the pose tracking (Figure~\ref{fig:no_depth}(c)).

% We constrain the object shape using the rendered depth maps, $\calD_i$ that are computed for the set of frames $\calS_i$ after each tracking step. The rendered-depth loss for the rays from previously tracked frames is defined as,
% \begin{equation}
%     \loss_\text{dep} = \sum_{\ray\in \{\calS_i\}_{i=0}^{t-1}} \big(\hat{d}(\ray)-\bar{d}(\ray)\big)^2,
% \end{equation}
% where, $\bar{d}(\ray)$ is the pre-computed depth of the ray and $\hat{d}(\ray)$ is the depth of the ray obtained using the rendering equation similar to Eq.~(\ref{eqn:rend_eqn}). Though $\bar{d}$ is not the accurate depth of the ray, it constrains the object shape from undergoing large deformations and provides a way for `remembering' the object shape reconstructed in the previous tracking steps. Our tracking loss thus constitutes both 2D and 3D terms and is defined as,
% \begin{equation}
%     \loss_\text{track} = \loss_\text{inc} + \loss_\text{dep}
% \end{equation}
% Figure~\ref{fig:with_depth} shows the normalized depth error and pose trajectories using the above tracking loss, $\loss_\text{track}$. The tracking is more stable with depth loss, $\loss_\text{dep}$.

% \begin{figure}[t]
%     \centering
%     \includegraphics[trim=50 0 55 8, clip, width=1\linewidth]{figures/method/depth_err_with_depth.pdf}
%     \caption{Rendered color images and normalized depth error between rendered depth and ground-truth depth for the frame shown in Figure~\ref{fig:no_depth} at different tracking steps when the 3D loss term $\loss_\text{dep}$ is used in tracking. The estimated and ground-truth trajectory of object pose is shown in the bottom row at different tracking steps. $\loss_\text{dep}$ results in more stable tracking while constraining the shape of the object.}
%     \label{fig:with_depth}
% \end{figure}

\subsection{Inter-Segment Optimization}
\label{sec:stitch}

Neighboring segments of the sequence contain overlapping frames whose poses are used to combine the segments. As the parts of object may be reconstructed in each segment with a different scale, the  poses in each segment are scale-normalized before combining two segments. Let $\campose_i^k =[\phi_i; t_i]$ be the rotation and translation of the camera for the $i^\text{th}$ frame in a segment, $k$ with $N_s$ frames, the unit-scale normalized pose of the camera is obtained as, $\hat{\campose}_i^k = \big[\phi_i; t_i/\frac{1}{N_s}\sum_i \|t_i\|\big]$. The camera poses of the overlapping frames in the segment $k$ are SE(3) transformed to align with frames in the neighboring segment, $\calN(k)$ using the matrix, $\campose_{k\rightarrow\calN(k)}$ obtained as,
\begin{equation}
    \campose_{k\rightarrow\calN(k)} = \arg\min_\campose \sum_i \|\campose\cdot\hat{\campose}_i^k-\hat{\campose}_i^{\calN(k)}\|_F,
\end{equation}
%
where, $\|\cdot\|_F$ denotes the Frobenius norm and the summation is over the set of overlapping frames. In practice, we observed that as less as a single overlapping frame is sufficient for combining the segments.

The cameras are initialized with the unit-scale normalized poses and the loss function defined in Eq.~(\ref{eq:first_loss}) is optimized to combine the segments. The network parameters, $\theta$ are initialized to reconstruct a sphere. Pairs of neighboring segments are iteratively combined until the object is reconstructed from the full sequence.

\subsection{Segmenting the Video Sequence}

Our choice of the algorithm for dividing the video sequence into multiple segments is driven by our tracking procedure explained in Section~\ref{sec:tracking_method} and to obtain accurate tracking within each segment. Recall that the regularization term (Eq.~(\ref{eq:reg_loss})) enforces near-plane surface reconstruction in the tracking step, $t=0$. We divide the video sequence into multiple segments and determine the tracking direction in each segment such that the observed object surface in the first frame of the segment is nearly-parallel to the image plane. We rely on object reprojection area in the image to determine the segment boundaries in the sequence and the tracking direction within the segment.

More specifically, frames with large object reprojection area contain object surfaces that are nearly-parallel to the image plane (see supplementary material for formal proof) and are thus good starting points for tracking. Figure~\ref{fig:seg_area} shows the plot of the object reprojection area through the sequence and sampled frames. The local maxima of the reprojection area are representative of the frames with large parallel object surface and are thus the segment-start boundaries. The local minima are chosen to be the segment-end boundaries as these are representative of the frames where the tracked object surface in the segment begins to self-occlude (see Figure~\ref{fig:seg_area}). We also set a threshold on the segment length to discard noisy segment boundaries and enforce 1-2 frame overlap between the segments.

\begin{figure}[t]
    \centering
    \includegraphics[trim=90 130 90 2, clip, width=1\linewidth]{figures/method/seg_area.pdf}
    \caption{Plot of object reprojection area for different frames in the sequence. The local maxima and minima of the reprojection area curve are used for determining the segment boundaries. The images of object at different parts of the sequence are shown in the inset.}
    \label{fig:seg_area}
\end{figure}


